Cyclical Long Memory: Decoupling, Modulation, and Modeling

A new model for general cyclical long memory is introduced, by means of random modulation of certain bivariate long memory time series. This construction essentially decouples the two key features of cyclical long memory: quasi-periodicity and long-term persistence. It further allows for a general cyclical phase in cyclical long memory time series. Several choices for suitable bivariate long memory series are discussed, including a parametric fractionally integrated vector ARMA model. The parametric models introduced in this work have explicit autocovariance functions that can be used readily in simulation, estimation, and other tasks.

==> Heuristic_arguments.tex <==


\section{Definitions of CLM} \label{appendix:acvf-spec-clm}
\normalsize

We shall first connect the definitions \eqref{eq:cycl-ACVF} and \eqref{eq:cyclical-spectrum} of CLM in Appendix \ref{app:subsec:spec-to-time} and \ref{app:subsec:time-to-spec}. We shall then derive the set of admissible cyclical phase parameters \eqref{eq:admiss-sets-def} in Appendix \ref{subsubsec:admis-phase}. Our approach will be partly heuristic, indicated by the notation $\simeq$ when that is the case. Our goal is to provide the reader with intuition behind the definitions and their constraints for CLM.

\subsection{From spectral to time domain} \label{app:subsec:spec-to-time}

We want to argue here that \eqref{eq:cyclical-spectrum} implies \eqref{eq:cycl-ACVF}, and also derive a relationship between various parameters. Choose small $\veps > 0$. Then, as $h \to \infty$,
\begin{equation} \label{eq:210}
\gamma_X(h) \simeq \Re \left[ \int_{\lambda_0 -\veps}^{\lambda_0+\veps} e^{ih \lambda} f(\lambda) d\lambda \right] = \Re \left[ \int_{\lambda_0 -\veps}^{\lambda_0} e^{ih \lambda} f(\lambda) d\lambda \right]+ \Re \left[\int_{\lambda_0 }^{\lambda_0+\veps} e^{ih \lambda} f(\lambda) d\lambda\right].
\end{equation}
We consider the two integrals in \eqref{eq:210} separately. First, note that, by using \eqref{eq:cyclical-spectrum},
\begin{equation*}
\begin{split}
    \int_{\lambda_0 -\veps}^{\lambda_0} e^{ih \lambda} f(\lambda) d\lambda &\simeq c_f^- \int_{\lambda_0 -\veps}^{\lambda_0} e^{ih \lambda} (\lambda_0 - \lambda)^{-2d}  d\lambda \\
    &= c_f^- e^{ih\lambda_0} \int_{0}^{\veps} e^{-ih z} z^{-2d}  dz \\
    &= c_f^- e^{ih\lambda_0} h^{2d-1} \int_{0}^{\veps h} e^{-ix} x^{-2d} dx,
\end{split}
\end{equation*}
where for the first equality we used the change of variables $ z \mapsto \lambda_0 - \lambda$ and for the second $x \mapsto hz$. Moreover, as $h \to \infty$,
\[
\int_{0}^{\veps h} e^{-ix} x^{-2d} dx \to \int_0^\infty e^{-ix} x^{-2d} dx = a_d e^{-i\psi_d}, 
\]
where $\psi_d \doteq \frac{(1-2d)\pi}{2}$ and $a_d \doteq \Gamma(1-2d)$ (see the formulas 3.761(4) and 3.761(9) in \cite{Graryz15} with $\mu = 1-2d, a = 1$). It follows that
\begin{equation} \label{eq:211}
\Re \left[ \int_{\lambda_0 -\veps}^{\lambda_0} e^{ih \lambda} f(\lambda) d\lambda \right] \simeq c_f^- a_d \cos(\lambda_0h-\psi_d) h^{2d-1}, \quad \text{as}\; h \to \infty. 
\end{equation}
Analogous calculations show that
\begin{equation} \label{eq:212}
\Re \left[ \int_{\lambda_0 }^{\lambda_0 + \veps} e^{ih \lambda} f(\lambda) d\lambda \right] \simeq c_f^+ a_d \cos(\lambda_0h+\psi_d) h^{2d-1}, \quad \text{as}\; h \to \infty. 
\end{equation}
By combining \eqref{eq:210}, \eqref{eq:211}, and \eqref{eq:212}, we get that, as $h \to \infty$,
\begin{equation} \label{eq:213}
\begin{split}
    \gamma_X(h) &\simeq c_f^- a_d \cos(\lambda_0h-\psi_d) h^{2d-1} + c_f^+ a_d \cos(\lambda_0h+\psi_d) h^{2d-1} \\
    &= a_d h^{2d-1}  \left[(c_f^+ + c_f^-)  \cos(\psi_d) \cos(\lambda_0 h) + (c_f^- - c_f^+)  \sin(\psi_d) \sin(\lambda_0h)\right] \\
    &= c_\gamma \cos(\lambda_0 h + \psi) h^{2d-1},
\end{split}
\end{equation}
where 
\begin{equation} \label{eq:cgamma-psi}
\begin{split}
    c_\gamma &\doteq a_d \sqrt{(c_f^+ + c_f^-)^2 \cos(\psi_d)^2 + (c_f^+ - c_f^-)^2 \sin(\psi_d)^2} = a_d \sqrt{((c_f^+)^2 + (c_f^-)^2 + 2 c_f^+ c_f^-\cos(2 \psi_d)^2} \\
    & \hspace{3cm} \psi \doteq  \arcsin \left( \frac{(c_f^+ - c_f^-) \sin(\psi_d)}{\sqrt{((c_f^+)^2 + (c_f^-)^2 + 2 c_f^+ c_f^-\cos(2 \psi_d)^2}}  \right).
\end{split}
\end{equation}
In particular, when $c_f^+ = c_f^- = c_f$, we get that
\begin{equation} \label{eq:cf-cf+cf}
    c_\gamma = 2 a_d c_f \cos(\psi_d), \quad \psi = 0.
\end{equation}
When, e.g., $c_f^+ > 0$ and $c_f^- = 0$, we get that
\begin{equation} \label{eq:cf-0}
    c_\gamma = a_d c_f^+, \quad \psi = \psi_d = \left( \frac{1}{2} - d \right) \pi.
\end{equation}
When $c_f^- > 0$ and $c_f^+ = 0$, we get that
\begin{equation} \label{eq:cf+0}
    c_\gamma = a_d c_f^-, \quad \psi = - \psi_d = - \left( \frac{1}{2} - d \right) \pi.
\end{equation}
\begin{remark}
    We note that the relation \eqref{eq:cyclical-spectrum} needs to be interpreted with caution when, for example, $c_f^+ = 0$. In this case, it states that
    \[
    f(\lambda) \sim 0, \quad \text{as}\; \lambda \to \lambda_0^+.
    \]
    In the arguments above, we treated this relation as $f(\lambda) \to 0$, as $\lambda \to \lambda_0^+$. The arguemnts extend to the case when $f(\lambda) \to $constant, as $\lambda \to \lambda_0^+$.
\end{remark}

\PZ{should I turn all the $\psi$'s to $\phi$'s for consistency?}

\subsection{From time to spectral domain} \label{app:subsec:time-to-spec}

We now turn to an argument deriving \eqref{eq:cyclical-spectrum} from \eqref{eq:cycl-ACVF}. We shall view \eqref{eq:cyclical-spectrum} as a relation for $f_X(\lambda_0 + \lambda)$ as $\lambda \to 0^+$ and $\lambda \to 0^-$. Consider first the case $\lambda \to 0^+$. Note that, by using \eqref{eq:cycl-ACVF},
\begin{align} 
    f_X(\lambda_0+ \lambda) &=  \frac{1}{2\pi} \left[ \gamma_X(0) + 2\sum_{h=1}^\infty \cos((\lambda_0+\lambda) h) \gamma_X(h)  \right] \simeq \frac{c_\gamma}{\pi} \sum_{h=1}^\infty \cos((\lambda_0+\lambda) h) \cos(\lambda_0 h+ \phi) h^{2d-1} \nonumber \\
    &= \frac{c_\gamma}{2\pi} \sum_{h=1}^\infty \bigg(\cos\big((\lambda+2\lambda_0) h + \phi\big) + \cos(\lambda h -\phi) \bigg)  h^{2d-1} \nonumber \\
    &= \frac{c_\gamma}{2\pi} \left[ \lambda^{-2d}  \sum_{h=1}^\infty  \cos(\lambda h -\phi)   (\lambda h)^{2d-1} \lambda + \sum_{h=1}^\infty \cos((\lambda+2\lambda_0) h + \phi) h^{2d-1}  \right] . \label{eq:acvf-spec-1}
\end{align}
Similar to Remark 2.2.18 in \cite{pipiras_taqqu_2017}, and from Formulas 3.761.4 and 3.761.9 of \cite{Graryz15}, we have for the first term in \eqref{eq:acvf-spec-1},
\begin{equation} 
\label{eq:acvf-spec-2}
\begin{split}
    \frac{c_\gamma}{2\pi} \lambda^{-2d} &\sum_{h=1}^\infty  \cos(\lambda h - \phi) (\lambda h)^{2d-1} \lambda \\
    &=  \frac{c_\gamma}{2\pi} \lambda^{-2d} \left[ \cos (\phi)  \sum_{h=1}^\infty  \cos(\lambda h) (\lambda h)^{2d-1} \lambda +  \sin(\phi)  \sum_{h=1}^\infty  \sin(\lambda h ) (\lambda h)^{2d-1} \lambda \right] \\
    &\simeq  \frac{c_\gamma}{2\pi} \lambda^{-2d}\left[ \cos(\phi) \int_0^\infty u^{2d-1} \cos(u) du + \sin(\phi) \int_0^\infty u^{2d-1} \sin(u)  du    \right] \\
    &= \frac{c_\gamma}{2\pi} \lambda^{-2d}\left[ \cos(\phi) \Gamma(2d) \cos(d\pi) + \sin(\phi) \Gamma(2d) \sin(d \pi)     \right] = c_f^+ \lambda^{-2d},
\end{split}
\end{equation}
with $c_f^+ \doteq \frac{c_\gamma}{2\pi} \Gamma(2d) \cos(d\pi - \phi)$. On the other hand, we expect for the second term in \eqref{eq:acvf-spec-1} that
\begin{equation} \label{eq:acvf-spec-3}
   \sum_{h=1}^\infty \cos((\lambda + 2\lambda_0)h + \phi) h^{2d-1} \simeq \sum_{h=1}^\infty \cos( 2\lambda_0 h + \phi) h^{2d-1} < \infty
\end{equation}
Carrying out similar calculations as $\lambda \to 0^-$ yields
\begin{equation}
    f_X(\lambda_0 + \lambda) \simeq \begin{cases}
        c_f^+ \lambda^{-2d}, & \lambda \to 0^+, \\
        c_f^- (-\lambda)^{-2d}, & \lambda \to 0^-,
    \end{cases}
\end{equation}
where
\begin{equation} \label{eq:cfpm-cgamma}
    c_f^\pm = \frac{c_\gamma}{2\pi} \Gamma(2d) \cos(d\pi \mp \phi).
\end{equation}
Note that \eqref{eq:cfpm-cgamma} is consistent with \eqref{eq:cf-cf+cf}, \eqref{eq:cf-0}, and \eqref{eq:cf+0}. It could also be derived from \eqref{eq:cgamma-psi} by solving for $c_f^+$ and $c_f^-$. \PZ{calculations are disgusting, should I check this?}.

\subsection{Set of admissible cyclical phases}
\label{subsubsec:admis-phase}

Since $c_f^+,c_f^- \ge 0$, note that \eqref{eq:cfpm-cgamma} yields
\[
-\frac{\pi}{2} \le d\pi - \phi \le \frac{\pi}{2}, -\frac{\pi}{2} \le  \phi - d\pi \le \frac{\pi}{2}
\]
so that, as stated in \eqref{eq:admiss-sets-def},
\[
\phi \in \cli_d = \left[\left(d - \frac{1}{2} \right)\pi  , \left(\frac{1}{2} - d\right) \pi \right].
\]
As in \eqref{eq:cf-0} and \eqref{eq:cf+0}, note again that the boundary values $\phi = \pm \left(\frac{1}{2}-d\right) \pi$ correspond to $c_f^\mp = 0$.



==> Old_Lemmas.tex <==
\begin{lemma} \label{lemma:second-order-cos}
    For $d \in (0,1/2)$, as $\om \to 0^+$,
    \[
    \sum_{k=1}^\infty \cos(k \om) k^{2d-1} = \om^{-2d} \Gamma(2d) \cos(\pi d) + R(\om),
    \]
    or with $p=1-2d \in (0,1)$
    \[
    \sum_{k=1}^\infty \cos(k \om) k^{-p} = \om^{p-1} \Gamma(1-p) \sin\left( p \frac{\pi}{2}\right) + R(\om),
    \]
    where the remainder term $R(\om) \to C \in \RR$ as $\om \to 0^+$. 
\end{lemma}


\begin{proof}
    Define, for fixed $p \in (0,1)$, $g(x) \doteq x^{2-p}$. Then, $g$ is clearly twice differentiable and it admits the following expansion
    \[
    \frac{\left(  1 + \frac{1}{k} \right)^{2-p} - 2 + \left(  1 - \frac{1}{k} \right)^{2-p}}{\frac{1}{k^2}} = g''(1) + O\left(\frac{1}{k^2}\right)
    \]
    or, since $g(1) = 1, g''(1) = (2-p)(1-p)$, 
    \begin{equation} \label{eq:power-law-1}
        k^{-p} = \frac{(k+1)^{2-p} - 2k^{2-p} + (k-1)^{2-p}}{(2-p)(1-p)}  + O\left(\frac{1}{k^{2+p}}\right).
    \end{equation}
    Then, in view of \eqref{eq:power-law-1},
    \begin{equation}
        \sum_{k=1}^\infty \cos(k\om) k^{-p} = \sum_{k=1}^\infty \cos(k\om) \frac{(k+1)^{2-p} - 2k^{2-p} + (k-1)^{2-p}}{(2-p)(1-p)} + \sum_{k=1}^\infty \cos(k \om) O\left(\frac{1}{k^{2+p}}\right),
    \end{equation}
    where, as $\om \to 0^+$,
    \begin{equation} \label{eq:c0-def}
       R_1(\om) \doteq  \sum_{k=1}^\infty \cos(k \om) O\left(\frac{1}{k^{2+p}}\right) \to \sum_{k=1}^\infty O\left(\frac{1}{k^{2+p}}\right) \doteq C.
    \end{equation}
    from DCT and the comparison test. This implies that
    \begin{equation}
        \sum_{k=1}^\infty \cos(k\om) k^{-p} 
        = \frac{2\pi}{(2-p)(1-p)} f_Z(\om)  +  R_1(\om)
    \end{equation}
    where $Z$ is a standard fractional Gaussian noise with Hurst parameter $H=1 - \frac{p}{2}$ and spectral density 
    \[
    f_Z(\om) = \left[ \frac{1}{2\pi} \sum_{k=-\infty}^\infty e^{-ik\om}  \frac{|k+1|^{2-p} - 2 |k|^{2-p} + |k-1|^{2-p}}{2}   \right].
    \]
    Let, as in Proposition 2.6.11 of \cite{pipiras_taqqu_2017},
    \[
    \left(c_2\left(1- \frac{p}{2}\right)\right)^2 \doteq \int_\RR |e^{ix} -1 |^2 |x|^{-p-3} \hat{B}(dx) = \frac{\pi}{(1-p/2)\Gamma(2-p) \sin\left((1-\frac{p}{2}) \pi \right)}= \frac{2\pi}{(2-p)(1-p)\Gamma(1-p) \sin\left(\frac{p}{2} \pi \right)}, 
    \]
    where $\hat B(dx)$ is a Hermitian Gaussian random measure with control measure $\EE |\hat{B}(dx) |^2 = dx$ and the second equality follows from display (2.6.10) of \cite{pipiras_taqqu_2017}. Then,
    \begin{equation}
    \begin{split}
        \sum_{k=1}^\infty \cos(k\om) k^{-p} &= \frac{2\pi}{(2-p)(1-p)} \frac{1}{c_2\left(1-\frac{p}{2}\right)^2} |1-e^{-i\om}|^2 \sum_{n=-\infty}^\infty |\om + 2\pi n|^{-1-2+p} + R_1(\om) \\
        &= \Gamma(1-p) \sin \left( \frac{p}{2} \pi  \right) |1-e^{-i\om}|^2 |\om|^{p-3} + R_1(\om) + R_2(\om) \\
        &= \Gamma(1-p) \sin \left( \frac{p}{2} \pi  \right) |\om|^{p-1} + R_1(\om) + R_2(\om) + R_3(\om),
    \end{split}
    \end{equation}
    where the first line follows from Proposition 2.8.1 of \cite{pipiras_taqqu_2017}, the second line from decomposing $\sum_{n=-\infty}^\infty = \sum_{n=0} + \sum_{n\neq0}$ and noticing that the latter sum converges uniformly in $\om$, and the third line from the remark that
    \[
    |1-e^{-i\om}|^2 = (1-\cos(\om))^2 + \sin^2(\om) = 4 \sin^2 \left( \frac{\om}{2} \right) = \om^2 + O(|\om|^4).
    \]
    Moreocer, notice that $R_2(\om), R_3(\om) = o(1)$. Thus by defining $R(\om) \doteq R_1(\om) + R_2(\om) + R_3(\om)$
    \[
    \sum_{k=1}^\infty \cos(k\om) k^{-p} = \Gamma(1-p) \sin \left( \frac{p}{2} \pi  \right) |\om|^{p-1} + R(\om).
    \]
    where $R(\om) \to C$ as $\om \to 0^+$, with $C$ specified in \eqref{eq:c0-def}.
\end{proof}

We now provide the corresponding result for power-law sine coefficients. Its proof relies on the theory of $G^*$ functions and an application of the Poisson summation formula, undertaken in Section 13 (Chpater 2) of \cite{zygmund_2003}.



\begin{lemma} \label{lemma:second-order-sin}
   For $d \in (0,1/2)$, as $\om \to 0^+$,
    \[
    \sum_{k=1}^\infty \sin(k \om) k^{2d-1} = \om^{-2d} \Gamma(2d) \sin(\pi d) + R(\om),
    \]
    or with $p=1-2d \in (0,1)$
    \[
    \sum_{k=1}^\infty \sin(k \om) k^{-p} = \om^{p-1} \Gamma(1-p) \cos\left( p \frac{\pi}{2}\right) + R(\om),
    \]
    where the remainder term $R(\om) \to C \in \RR$ as $\om \to 0^+$. 
\end{lemma}


\begin{proof}
    We will show the claim in its latter formulation. Define, for $0 < \om < 2\pi$, the periodic function 
   \begin{equation} \label{eq:Psi-p-def}
   \begin{split}
       \Psi_p(\om) &\doteq \lim_{n \to \infty} \frac{2\pi}{\Gamma(p)} \left( \om^{p-1} + (\om+2\pi)^{p-1} + \dots + (\om+2\pi n)^{p-1} - \frac{(2\pi)^{p-1}}{p}n^p \right) \\
       &= \frac{2\pi}{\Gamma(p)}  \om^{p-1} + \lim_{n \to \infty} \frac{2\pi}{\Gamma(p)} \left(  (\om+2\pi)^{p-1} + \dots + (\om+2\pi n)^{p-1} - \frac{(2\pi)^{p-1}}{p}n^p \right).
    \end{split}
   \end{equation}
   Note that the limit in the first line of \eqref{eq:Psi-p-def} exists uniformly in $\veps < \om < 2\pi$ for all $\veps > 0$, and that the limit in the second line exists uniformly for all $0 \le \om \le 2\pi$ (see, e.g., the discussion above (13.11) in Chapter 2 of \cite{zygmund_2003}). Moreover, from Theorem 13.7 (Chapter 2) of \cite{zygmund_2003}, the Fourier series for this function are known
   \begin{equation}
       \Psi_p(\om) \sim \sum_{\substack{k=-\infty \\ k\neq 0}}^\infty \frac{e^{-\frac{1}{2} \pi i p \text{sign}(k)}}{|k|^p} e^{ik\om}
   \end{equation}
   and hence the following identity holds, for $0 < \om <2\pi$:
   \begin{equation} \label{eq:Psi-p-sin-1}
       \Psi_p(\om) - \Psi_p(-\om) = 4 \sin \left( \frac{1}{2} \pi p  \right) \sum_{k=1}^\infty \frac{\sin(k \om)}{k^p}.
   \end{equation}
   On the other hand, due to \eqref{eq:Psi-p-def}, as $\om \to 0^+$,
   \begin{equation} \label{eq:Psi-p-sin-2}
       \Psi_p(\om) - \Psi_p(-\om) = \frac{2\pi}{\Gamma(p)}  \om^{p-1} + R_1(\om),
   \end{equation}
    where
    \begin{equation}
          R_1(\om) \doteq \lim_{n \to \infty} \frac{2\pi}{\Gamma(p)} \left( (\om+2\pi)^{a-1} + \dots + (\om+2\pi n)^{a-1} - \frac{(2\pi)^{p-1}}{p}n^p \right) + \Psi_a(2\pi -\om),
    \end{equation}
    and for $0 \le \om \le \pi$, $R_1(\om)$ exists. By comparing \eqref{eq:Psi-p-sin-1} and \eqref{eq:Psi-p-sin-2} and by defining $R(\om) \doteq R_1(\om) \left(4 \sin \left( \frac{1}{2} \pi p  \right) \right)^{-1}$,
    \begin{equation}
        \sum_{k=1}^\infty \frac{\sin(k \om)}{k^p} = \om^{p-1} \Gamma(1-p) \cos \left( p \frac{\pi}{2} \right) + R(\om),
    \end{equation}
    where the equality holds in view of the identity $\Gamma(p) \Gamma(1-p) = \frac{\pi}{\sin(\pi p)}$. Moreover, note that $R(\om) \to R(0) = C \in \RR$ as $\om \to 0^+$.
    \end{proof}

==> Old_thoughts.tex <==
% Its matrix-valued ACVF $\gamma_X(h) \in \RR^{2\times 2}$ and its spectral density $f_X(\lambda) \in \CC^{2 \times 2}$ (assuming it exists and under mild conditions) are given by
% \[
% \gamma_X(h) = \EE  X_h X_0^T -  \EE X_h \EE X_0^T, \quad \text{and} \quad f_X(\lambda) = \frac{1}{2\pi} \sum_{j \in \ZZ} e^{-ij\lambda} \gamma_X(j)
% \]
% respectively. We will use $\gamma_X$ and $\gamma^X$ indistinguishably. $\gamma_X$ need not have symmetric values and $f$ can have complex-valued entries in general. For the ACVF of a bivariate stationary process $(X_n^1,X_n^2) \in \RR^2$, we denote by $\gamma^X_{jk}(h)$ or $\gamma_{X^j,X^k}(h)$ the $(j,k)-$th element of $\gamma_X$ at lag $h$. 
% We recall that a bivariate second-order stationary time series is LM if one of the following two, non-equivalent (in general) conditions is satisfied:
% \begin{enumerate}
%     \item If for some $R(h), R \in \RR^{2\times 2}$ with $R(h) \sim R$ as $h \to \infty$ and $R_{11}, R_{22} \neq 0$, the ACVF can be written 
% \[ 
% \gamma_X(h) = (R_{jk}(h)h^{d_j + d_k -1})_{j,k=1,2},
% \]
% with $d_j \in (0,1/2),j=1,2$. 

% \item
% If the spectral density matrix function satisfies
% \begin{equation} \label{eq:spec-biv-general}
% f(\lambda) = (G_{jk} (\lambda) \lambda^{-(d_j + d_k)})_{j,k=1,2}
% \end{equation}
% with $G(\lambda) \sim G$ as $\lambda \to 0^+$, where $G(\lambda),G \in \CC^{2 \times 2}$ are Hermitian symmetric, and non-negative definite matrix functions and $G = (g_{jk} e^{i \om_{jk}})_{j,k=1,2}$ with $g_{ij} \in \RR, g_{11}, g_{22} \neq 0$, and $\om_{jk} \in (-\pi,\pi]$.
% \end{enumerate}
% Under mild conditions on the matrices $R$ and $G$, the above definitions are equivalent (see Proposition 2.1 of \cite{KecPi15}). These conditions will always be met for the bivariate series considered in the sequel and so we will use them indistinguishably.  


% Notice that in the case of bivariate LM, one also has a parameter $\om$ called the \textit{bivariate phase parameter}\footnote{in \cite{KecPi20}, $\phi$ was used to denote the bivariate phase. Here, we reserve $\phi$ for the cyclical phase and use $\om$ instead.}, that controls the assymetry of the process in large time lags. We emphasize here the distinction between the cyclical phase parameter introduced in \eqref{eq:cycl-ACVF} and the phase parameter related to a bivariate time series. The phase parameter is explicitly obtained by the asymptotics of the spectral density of a bivariate LM series in the form
% \begin{equation} \label{eq:bivariate-form-spectral}
% f(\lambda) \sim \begin{pmatrix}
% g_{11} |\lambda|^{-2d_1} & g_{12} |\lambda|^{-d_1 - d_2} e^{-i \text{sign}(\lambda) \om} \\
% g_{21} |\lambda|^{-d_1 - d_2} e^{i \text{sign}(\lambda) \om} & g_{22} |\lambda|^{-2d_2}
% \end{pmatrix}, \quad \text{as} \; \lambda \to 0,
% \end{equation}
% where $G = [g_{ij}]_{i,j=1,2}$. The case $\om = 0$ corresponds to series that exhibit symmetry (time-reversibility).



% \subsection{Notation and Terminology}

% Let $\mathbb{F} = \mathbb{R}$ or $\mathbb{F} = \mathbb{C}$  and for $n,m \in \NN$, denote by $\mathbb{F}^{n \times m}$ the set of $n\times m$ matrices, where each component takes values in $\mathbb{F}$. For matrices $A_n,A \in \mathbb{F}^{n \times k}$, the transpose (resp. Hermitian transpose) will be denoted by $A^T$ (resp. $A^*$), and we write $A_n \sim A$ to denote coordinatewise convergence in $\mathbb{F}$, equipped with its usual topology. Throughout this work, we let $\{\veps_n\}_{n \in \NN}$ denote a $\RR^2$-valued White Noise (WN) sequence defined on some silent probability space $(\Omega,\clf,\PP)$ with normalized means ($\EE \veps_n = 0$ for all $n \in \NN$) and variance ($\EE \veps_n \veps_n^T = I$), where $I$ will be reserved for the identity element of $\RR^{2\times 2}$. For a complex number $c \in \mathbb{C}$, denote by $\Re(c)$ (resp. $\Im(c)$) the real (resp. imaginary) part of $c$. Throughout this work, we will write $B$ to denote the backshift operator. In this study, we will say that a process is stationary if it is weakly stationary. For a time series $\{Z_n\}_{n \in \ZZ}$, its (discrete-time) Hilbert transform is a time series denoted by $\{\clh[Z_n]\}_{n \in \ZZ}$ defined as
% \[
% \clh[Z_n] \doteq \sum_{i \in \ZZ} h_i Z_{n-i}, \quad h_j \doteq \begin{cases}
%     0 & \text{if } j \text{ is even} \\
%     \frac{2}{\pi j} & \text{if } j \text{ is odd}
% \end{cases}.
% \]


$ \quad \Psi_j \doteq A_j |j|^{d-1}$
% Modulation of stochastic processes is a fundamental tool originating from signal processing in egineering \cite{Pap83}, and was initially motivated by representing a stochastic process as an amplitude modulation and frequency modulation signal by using suitable transformations. In this Section, we describe how random modulation can be used to represent CLM series with the two components of a bivariate LM series.


% Notice that a particularly intriguing feature of CLM in \eqref{eq:cycl-ACVF} is the product of the two terms $\cos(\lambda_0 h + \phi)$ and $h^{2d-1}$. The second one is associated with LM series, while the first seems to suggest some modulation of the latter by $e^{i \lambda_0 h}$. Indeed, take two independent copies of LM series \PZ{with the same ACVF at all lags} $Y^{(1)} = \{Y_{1,n}\}_{n \in \ZZ}$ and $Y^{(2)} = \{Y_{2,n}\}_{n \in \ZZ}$ with ACVF satisfying $\gamma_Y (h) \sim c_\gamma h^{2d-1}$, and set
% \begin{equation}\label{eq:cycl-constr-basic}
%     X_n \doteq \cos(\lambda_0 n) Y_{1,n} + \sin(\lambda_0n) Y_{2,n}, \quad n \in \ZZ.
% \end{equation}
% It is straightforward to check that $\{X_n\}_{n \in \ZZ}$ is a \PZ{weakly} stationary time series with ACVF satisfying
% \[
% \gamma_X(h) = \cos(\lambda_0 h) \gamma_Y(h) \sim  c_\gamma \cos(\lambda_0 h) h^{2d-1} ,
% \]
% that is, it exhibits CLM in the sense of \eqref{eq:cycl-ACVF} and \eqref{eq:cyclical-spectrum} with $\phi = 0$; cf. \eqref{eq:cycl-phi-0} and \eqref{eq:cyclical-spectrum}. Note that the construction \eqref{eq:cycl-constr-basic} decouples the cyclical and long memory properties by using two LM series, and paves an easy way for building CLM models. We are not aware of other works considering the construction \eqref{eq:cycl-constr-basic} for CLM series.

% The construction \eqref{eq:cycl-constr-basic} is straightforward, but note that it leads to CLM \eqref{eq:cycl-ACVF} with $\phi = 0$ only. Much of this study was motivated by the question:
% \[
% \text{are there constructions of the type \eqref{eq:cycl-constr-basic} leading to CLM \eqref{eq:cycl-ACVF} with artbitrary }\phi?
% \]
% Indeed, this can be achieved by imposing the dependence structure described in \eqref{Property1} on the LM series $Y^{1}$ and $Y^{2}$. This approach leads to explicit ACVF and spectral density of the resulting CLM series $\{X_n\}_{n \in \ZZ}$ that can be used easily in downstream tasks like simulation, estimation, and others. As we discuss further below, this is advantageous over many existing CLM models. 
% In fact, we are not aware of any parametric CLM models with $\phi \neq 0$ either.


% With a general construction as in \eqref{eq:cycl-constr-basic} capturing \eqref{eq:cycl-ACVF} and \eqref{eq:cyclical-spectrum}, we shall also consider parametric models for the bivariate series $Y^n = \{  Y_{1,n},Y_{2,n} \}_{n \in \ZZ}$. 


% Constructing time series that satisfy Property \eqref{Property1} is not a trivial task. Consider a bivariate time series $\{Z_n\}_{n \in \ZZ}$ in its linear representation

where $\Psi, A_j \in \RR^{2 \times 2}$. Further assume that, with $A^+,A^- \in \RR^{2\times 2}$
\begin{equation} \label{eq:A+A-conv}
    A_j \to A^+, \;\text{as}\; j \to + \infty, \quad \text{and} \quad A_j \to A^-, \;\text{as}\; j \to - \infty.
\end{equation}
Together with \eqref{Property1}, this says that, for some $a_0,a_1 \in \RR$,
\begin{equation} \label{eq:A+A-format}
A^+ = \begin{pmatrix}
    a_0 & a_1 \\
    -a_1 & a_0
\end{pmatrix}, \quad
A^- = \begin{pmatrix}
    a_0 & -a_1 \\
    a_1 & a_0
\end{pmatrix},
\end{equation}
Moreover, if the ACVF of $Y$ is as in \eqref{eq:ACVF-Y}, then \eqref{Property1} implies that, for some constants $a,b \in \RR$,
\begin{equation} \label{eq:R-Y} \tag{P2}
R(h) \sim R \doteq
\begin{pmatrix} 
a & -b \\
b & a
\end{pmatrix},\; \text{as} \; h \to \infty.
\end{equation}
Restrictions on the constants $a,b$ become apparent in the frequency domain, and their implication to the set of admissible cyclical phases $\cli_d$ will be discussed in Subsection \ref{subsubsec:admis-phase}. 

The discussion above suggests some sufficient conditions on the coefficients $\{ \Psi_n \}_{n \in \NN_0} $ that guarantee the desired properties. We state these in the following Lemma.




\begin{remark} \label{rmk:linear-repr-unique}
Note that the conditions for Theorem \ref{thm:linear-repr-biv} are sufficient for a linear representation to satisfy Property \eqref{Property1}, but not necessary. For instance, Theorem \ref{thm:linear-repr-biv} is also true if
     \[
    A_j =
    \begin{cases} 
      A_{+,j} \doteq \begin{pmatrix}
          a_{0,j} &  a_{1,j} \\
          -a_{1,j} &  a_{0,j}
      \end{pmatrix}  & j \ge l+1 \\
      A_{-,j} \doteq \begin{pmatrix}
          a_{0,j} &  -a_{1,j} \\
          a_{1,j} &  a_{0,j}
      \end{pmatrix} & j \le l
   \end{cases}
   \]
    for some $l \in \ZZ$. 
    
    % The construction of a time series that preserves this property, but is substantially different than the one presented in Theorem \ref{thm:linear-repr-biv} is an problem for which we do not have an answer.
\end{remark}


% We now investigate the set of admissible phases $\cli_d$ in the frequency domain. By Proposition 2.1 of \cite{KecPi15}, we see that a bivariate series $\{Y_n\}_{n \in \ZZ}$ with asymptotic ACVF given in \eqref{eq:R-Y} and $d_1=d_2=d$, must have spectral density as in \eqref{eq:spec-biv-general}, with
% \begin{equation} \label{eq:Y-G}
% G = \frac{\Gamma(2d)}{\pi} 
% \begin{pmatrix} 
% a \cos(\pi d) & i b \sin(\pi d) \\
% -i b \sin(\pi d) & a \cos(\pi d)
% \end{pmatrix}.
% \end{equation}
% Clearly $G$ is Hermitian, and such a series $\{Y_n\}_{n \in \ZZ}$ exists only if $G$ is positive semi-definite. By Sylvester's criterion, this implies that $a \ge 0$ (by the $1 \times 1$ principal minor) and also
% \[
% a^2 \cos^2 (\pi d) + i^2 b^2 \sin^2 (\pi d) \ge 0,
% \]
% or restated,
% \begin{equation} \label{eq:adm-set-1}
% a^2 \cos (\pi d) \ge b^2 \sin (\pi d).
% \end{equation}
% Now we consider two different cases. First, let $a,b \ge 0$, then \eqref{eq:adm-set-1} says that, by writing $a = c \cos(\phi), b = c \sin(\phi)$ with $\phi$ as in \eqref{eq:phi-def} and $c \doteq \sqrt{a^2 + b^2}$, we have that $\phi \in [0,\pi/2]$. Moreover, \eqref{eq:adm-set-1} implies
% \[
% c \cos(\phi) \cos(\pi d) - c \sin(\phi) \sin(\pi d) \ge 0,
% \]
% which then says that necessarily $\phi \in [0, \pi (\frac{1}{2} - d)]$. Now assume that $a \ge 0$ and $b< 0$, and so $\phi \in [-\pi/2,0)$. Similar calculations as before show that
% \[
% c \cos(\phi) \cos(\pi d) + c \sin(\phi) \sin(\pi d) \ge 0,
% \]
% and so $\phi \in [\pi(d-\frac{1}{2}),0)$. Overall the above statements say that by using the construction in this work, the admissible set for $\phi$ in \eqref{eq:cycl-ACVF} -parametrized by $d$- is the interval 
% \begin{equation} \label{eq:admissible-set}
% \cli_d = \left[\pi \left(d - \frac{1}{2}\right), \pi\left(\frac{1}{2}-d\right)\right].
% \end{equation}

% \begin{remark}
%     Here we have identified the admissible values for the cyclical phase $\phi$ with our method of constructing CLM through a bivariate series $\{Y_n\}_{n \in \ZZ}$. In fact, it will become clear in Section \ref{subsec:RM-insights} that every CLM with an admissible cyclical phase $phi$ can be represented as a random modulation of a bivariate LM series.
% \end{remark}

Assume that, with $A^+,A^- \in \RR^{2\times 2}$
\begin{equation} \label{eq:A+A-conv}
    A_j \to A^+, \;\text{as}\; j \to + \infty, \quad \text{and} \quad A_j \to A^-, \;\text{as}\; j \to - \infty.
\end{equation}
Together with \eqref{Property1}, this says that, for some $a_0,a_1 \in \RR$,
\begin{equation} \label{eq:A+A-format}
A^+ = \begin{pmatrix}
    a_0 & a_1 \\
    -a_1 & a_0
\end{pmatrix}, \quad
A^- = \begin{pmatrix}
    a_0 & -a_1 \\
    a_1 & a_0
\end{pmatrix},
\end{equation}
Moreover, if the ACVF of $Y$ is as in \eqref{eq:ACVF-Y}, then \eqref{Property1} implies that, for some constants $a,b \in \RR$,
\begin{equation} \label{eq:R-Y} \tag{P2}
R(h) \sim R \doteq
\begin{pmatrix} 
a & -b \\
b & a
\end{pmatrix},\; \text{as} \; h \to \infty.
\end{equation}
Restrictions on the constants $a,b$ become apparent in the frequency domain, and their implication to the set of admissible cyclical phases $\cli_d$ will be discussed in Subsection \ref{subsubsec:admis-phase}. 


\begin{remark}
    We remark that the limiting matrix in \eqref{eq:R-Y} corresponds to series with bivariate phase $\om = \pi/2$ or $-\pi/2$ (see, e.g., (30) in \cite{KecPi15}) \PZ{Here we are using a heuristic since the formula is $\arctan(\infty)$. How do we justify this?}. From Proposition 2.1 of \cite{KecPi20} we are in the boundary case $|c|=1$, and so the simplified models considered there cannot assume the phase that is required for \eqref{Property1} to be satisfied.
\end{remark}


Consider a bivariate, weakly stationary LRD stochastic process $Y_n =(Y_n^{(1)},Y_n^{(2)}) \in \RR^2 $ with memory parameters $d \doteq d_1=d_2 \in (0,1/2)$ and matrix ACVF given by
\begin{equation}
\label{eq:ACVF-Y}
\gamma^Y(h) = (R_{jk}(h) h^{d_j+d_k -1})_{j,k=1,2} = (R_{jk}(h) h^{2d-1})_{j,k=1,2}.
\end{equation}

% The construction of a parametric series satisfying \eqref{Property1} will be postponed to Section \ref{subsec:bivar-constr}. Define 
% \begin{equation} \label{eq:cycl-constr-basic} 
% X_n \doteq \cos(\lambda_0 n) Y_n^{(1)} + \sin(\lambda_0 n) Y_n^{(2)}, \quad n \in \ZZ,
% \end{equation}
and so for the series $\{X_n\}_{n \in \ZZ}$ we have the following Proposition.

Now we introduce short-range effects to the VARFIMA Model introduced before, by adding a $q$-th order moving average component to the two-sides representation of Lemma \ref{thm:linear-repr-biv}. Define
\begin{equation} \label{eq:ma-def}
    \Theta(x) \doteq \sum_{j=1}^q \Theta_j x^j, \quad \Psi(x) \doteq \sum_{j \in \ZZ} \Psi_j x^j
\end{equation}
where $\Theta_j = \diag(\theta_j,\theta_j) \in \RR^{2\times2}$, with $\theta_j \in \RR$ for $j=1,\dots,q$, and $\Psi_j$ are as in \eqref{eq:Zn}. We have the followin result

\begin{lemma} \label{lem:tilde-zn}
    Let $\{ \tilde Z \}_{n \in \ZZ}$ be a linear time series given by 
    \[
    \tilde Z_n = \Psi(B) (I + \Theta(B)) \veps_n 
    \]
    where $\Psi_j$ is defined in \eqref{eq:Zn}, \eqref{eq:ma-def}, \eqref{eq:A+A-conv},\eqref{eq:A+A-general} and $\Theta(x)$ in \eqref{eq:ma-def}. Then, $\tilde Z_n$ satisfies \eqref{Property1}. Moreover, the moving average and linear series expansion components commute, i.e. $\tilde Z_n =  (I + \Theta(B)) \Psi(B) \veps_n$ .
\end{lemma}

\begin{proof}
    We write
\begin{equation}
\begin{split}
    \tilde Z_n = \Psi(B) (I + \Theta(B)) \veps_n &= \dots + \Psi_{-2}\left(\veps_{n-2} + \sum_{j=1}^q \Theta_j \veps_{n-2-j} \right) + \Psi_{-1}\left(\veps_{n-1} + \sum_{j=1}^q \Theta_j \veps_{n-1-j} \right) \\
    &+ \Psi_0\left(\veps_{n} + \sum_{j=1}^q \Theta_j \veps_{n-j} \right) + \Psi_1 \left(\veps_{n+1} + \sum_{j=1}^q \Theta_j \veps_{n+1-j} \right) + \dots \\
    &= \sum_{j \in \ZZ} \left( \Psi_j + \sum_{i=1}^q \Psi_{j+i} \Theta_i   \right) \veps_{n-j} 
    \doteq \sum_{j \in \ZZ} \tilde \Psi_j \veps_{n-j},
\end{split}
\end{equation}
where after performing the calculations, we have
    \[
    \tilde \Psi_j =
    \begin{cases} 
       \begin{pmatrix}
          a_{0,j} + \sum_{l=1}^q a_{0,j+l} \theta_l &  -a_{1,j} - \sum_{l=1}^q a_{1,j+l} \theta_l \\
          a_{1,j} + \sum_{l=1}^q a_{1,j+l} \theta_l &  a_{0,j} + \sum_{l=1}^q a_{0,j+l} \theta_l
      \end{pmatrix}  & j \le -q \\
      \begin{pmatrix}
          a_{0,j} + \sum_{l=1}^q a_{0,j+l} \theta_l &  -a_{1,j} - \sum_{l=1}^{|j|} a_{1,j+l} \theta_l + \sum_{l= |j|+1}^q a_{1,j+l} \theta_l \\
          a_{1,j} + \sum_{l=1}^{|j|} a_{1,j+l} \theta_l - \sum_{l= |j|+1}^q a_{1,j+l} \theta_l &  a_{0,j} + \sum_{l=1}^q a_{0,j+l} \theta_l
      \end{pmatrix}  &  -q+1 \le j \le -1 \\
      \begin{pmatrix}
          a_{0,j} + \sum_{l=1}^q a_{0,j+l} \theta_l &  +a_{1,j} +\sum_{l=1}^q a_{1,j+l} \theta_l \\
          -a_{1,j} - \sum_{l=1}^q a_{1,j+l} \theta_l &  a_{0,j} + \sum_{l=1}^q a_{0,j+l} \theta_l
      \end{pmatrix}  & j \ge 0
   \end{cases}.\]
It is now clear that $\{\tilde \Psi_j\}_{j \in \ZZ}$ meets the conditions of Lemma \ref{thm:linear-repr-biv} and so the conclusion follows. Analogous calculations reveal that $(I + \Theta(B)) \Psi(B) \veps_n = \Psi(B) (I + \Theta(B)) \veps_n$.
\end{proof}

\begin{remark}
    Lemma \ref{lem:tilde-zn} says
    that \eqref{Property1} is closed under a certain type of moving average transformation of the linear series representation in \eqref{eq:Zn}.
\end{remark}

The following result provides a parametric VARFIMA$(0,D,q)$ model that satisfies \eqref{Property1}. Its proof is a trivial application of \ref{lem:tilde-zn} and \ref{thm:constr} and so we ommit it.

\begin{corollary} \label{corrol:VARFIMA-PD0}
    Let $\{Z_n\}_{n \in \ZZ}$ be given by
    \[
    Z_n = (I + \Theta(B)) \Delta(B) \veps_n,
    \]
    where $\Theta(x)$ is given in \eqref{eq:ma-def} (with $\Theta_j = \diag(\theta_j,\theta_j)$ and $\Delta(x)$ is given in \eqref{eq:Yn}.
\end{corollary}


Moreover, for each fixed $ \lambda_0 \in (0,\pi)$, we can choose some $\lambda > 0$ with $\lambda + 2\lambda_0 < 2\pi$. Hence, by applying Dirichlet's test with $a_h \doteq h^{2d-1}, b_h \doteq \cos(( \lambda+ 2\lambda_0)h)$, as $\lambda \to 0^+$
\begin{equation} \label{eq:acvf-spec-3}
\begin{split}
\lim_{\lambda \to 0^+} \sum_{h=1}^\infty \cos((\lambda + 2\lambda_0)h + \phi) h^{2d-1} &=   \cos(\phi) \lim_{\lambda \to 0^+} \sum_{h=1}^\infty \cos((\lambda + 2\lambda_0)h ) h^{2d-1}   \\
&- \sin(\phi) \lim_{\lambda \to 0^+} \sum_{h=1}^\infty \cos((\lambda + 2\lambda_0)h ) h^{2d-1}   
< \infty,
\end{split}
\end{equation}
Now by observing that the term in \eqref{eq:acvf-spec-3} is $O(\lambda^{-2d})$ and by \eqref{eq:acvf-spec-1} and \eqref{eq:acvf-spec-2}, we have that, as $\lambda \to 0^+$,
\[
f_X(\lambda_0+\lambda) \sim c_f^+ \lambda^{-2d}, \quad \text{or equivalently} \quad f_X(\lambda) \sim c_f^+ (\lambda - \lambda_0)^{-2d}.
\]
We investigate now the asymptotics of the form $f_X(\lambda_0+\lambda)$, as $\lambda \to 0^-$. Then, calculation analogous to \eqref{eq:acvf-spec-3} show that, as $\lambda \to 0^+$
\[
f_X(\lambda_0 - \lambda) \sim \frac{c_\gamma}{2\pi} \left[ \lambda^{-2d}  \sum_{h=1}^\infty  \cos(\lambda h +\phi)   (\lambda h)^{2d-1} \lambda + \sum_{h=1}^\infty \cos((2\lambda_0 - \lambda) h + \phi) h^{2d-1}  \right].
\]
Furthermore, as in \eqref{eq:acvf-spec-1},
\begin{equation*} 
        \frac{c_\gamma}{2\pi} \lambda^{-2d} \sum_{h=1}^\infty  \cos(\lambda h + \phi) (\lambda h)^{2d-1} \lambda \sim c_f^- \lambda^{-2d},
\end{equation*}
with $c_f^- \doteq \frac{c_\gamma}{2\pi} \Gamma(2d) \cos(d \pi + \phi)$. By the last two displays and a further application of Dirichlet's test, as $\lambda^+,$
\[
f_X(\lambda_0 - \lambda) \sim c_f^- \lambda^{-2d}, \quad \text{or equivalently} \quad f_X(\lambda) \sim c_f^- (\lambda_0 - \lambda)^{-2d}.
\]
In particular \eqref{eq:cycl-phi-0} follows.


In this Section of the Appendix, we demonstrate how the set of admissible phases $\cli_d$ below \eqref{eq:cycl-ACVF} is derived, and show that every $\phi \in \cli_d$ is, in fact, attainable with the random modulation construction.

Remark that, from the calculations in the previous section of the Appendix, we have the following formulas relating the coefficients of the time and the spectral domain of a CLM series
\[
c_f^+ = \frac{c_\gamma}{2\pi}\Gamma(2d) \cos(d\pi - \phi), \; c_f^- = \frac{c_\gamma}{2\pi}\Gamma(2d) \cos(d\pi + \phi).
\]


\begin{proof}
    Define the matrix (resp. vectors)
    \[
    M \doteq \begin{pmatrix}
        \cos(\lambda_0) & \sin(\lambda_0) \\
        -\sin(\lambda_0) & \cos(\lambda_0)
    \end{pmatrix}, \quad 
    v_n \doteq \begin{pmatrix}
        \cos(\lambda_0 n) & \sin(\lambda_0 n)
    \end{pmatrix}^T   \quad
    v_0 \doteq \begin{pmatrix}
        1 & 0
    \end{pmatrix}^T
    \]
    and observe that the following identities hold
    \[
    M^j =
    \begin{cases}
        \begin{pmatrix}
        \cos(\lambda_0 j) & \sin(\lambda_0 j) \\
        -\sin(\lambda_0 j) & \cos(\lambda_0 j) 
    \end{pmatrix} & \text{if }j \ge 1 \\
        \begin{pmatrix}
        \cos(\lambda_0 j) & -\sin(\lambda_0 j) \\
        \sin(\lambda_0 j) & \cos(\lambda_0 j) 
    \end{pmatrix} & \text{if }j \le -1
   \end{cases},
   \quad
   v_j^T =  \begin{cases}
       v_0^T M^j & j \ge 1, \\
       (M^j v_0)^T = v_0^T (M^j)^T & j \le 0.
   \end{cases}
    \]
Recall the expansion of $Y_n$ in \eqref{eq:Yn}--\eqref{eq:def-Q+-}. Then, the last two displays imply that
    \begin{equation}
    \begin{split}
        X_n &= v_n^T Y_n = v_0^T M^n \left[ \sum_{j=0}^\infty c_{d,j} Q_+ \veps_{n-j} +  \sum_{j=0}^\infty c_{d,j} Q_- \veps_{n+j} \right] \\
        &=   \sum_{j=0}^\infty c_{d,j} v_0^T M^j M^{n-j} Q_+ \veps_{n-j} +  \sum_{j=0}^\infty c_{d,j} v_0^T M^{-j} M^{n+j} Q_- \veps_{n+j} \\
        &=   \sum_{j=0}^\infty c_{d,j} v_0^T M^j \tilde \veps_{n-j} +  \sum_{j=0}^\infty c_{d,j} v_0^T M^{-j} \tilde \veps_{n+j}  
        % &= v_n^T \sum_{j=-\infty}^\infty \tilde Q_j \veps_{n-j} = \sum_{j=-\infty}^0 v_0^T M^j \tilde \veps_{n-j} + \sum_{j=1}^\infty (M^j v_0)^T \tilde \veps_{n-j} \\
        % &= \sum_{j \in \ZZ} \cos(\lambda_0 j) \tilde \veps_{n-j}^{(1)} + \sum_{j \in \ZZ} \sin(\lambda_0 j) \tilde \veps_{n-j}^{(2)} 
    \end{split}
    \end{equation}
where 
\[
\tilde \veps_{n-j} =  M^{n-j} Q_+ \veps_{n-j}, \veps_{n+j} = M^{n+j} Q_- \veps_{n+j} 
\]
\[
\tilde \veps_{n-j} \doteq M^{n-j} \tilde Q_j \veps_{n-j}.
\]
We remark that the two components of $\tilde Q_j \veps_{n-j}$ are uncorrelated and Gaussian, and so, by the orthogonality of $M^j$, $\tilde \veps_{j}$ is a Gaussian white noise sequence with 
\[
var(\tilde \veps_{n-j}) = \EE\left( \tilde \veps_{n-j} \tilde \veps_{n-j}^T   \right) = \EE \left( M^{n-j} \tilde Q_j \veps_{n-j} \veps_{n-j}^T \tilde Q_j^T (M^{n-j})^T  \right) = \EE \left( \tilde Q_j \veps_{n-j} \veps_{n-j}^T \tilde Q_j^T  \right) = (q_0^2 + q_1^2) \text{Id}.
\]
This concludes the proof.
\end{proof}


We consider the following extension of a CLM series in the spectral domain, proposed in \cite{Arteche20003}
\begin{equation} \label{eq:cyclical-spectrum-assymetry-memory}
 f_X(\lambda) \sim 
 \begin{cases}
       c_f^+ (\lambda - \lambda_0)^{-2d_1}, &\quad\text{as}\; \lambda \to \lambda_0^+\\
       c_f^- (\lambda_0 - \lambda)^{-2d_2}, &\quad\text{as}\; \lambda \to \lambda_0^-
 \end{cases},
\end{equation}
where $c_f^+,c_f^- > 0$, and $d_1,d_2 \in \left(0,\frac{1}{2}\right)$. It turns out that constructing a series exhibiting this spectral density with random modulation techniques is also straightforward.

Take two independent bivariate series $\{ (Y_{1,l},Y_{2,l}) \}_{l \in \ZZ}$ and $\{ (\tilde Y_{1,l},\tilde Y_{2,l}) \}_{l \in \ZZ}$ with LM parameters $d_1,d_2 \in \left(0,\frac{1}{2}\right)$ such that, if we define two CLM series by
\begin{equation} \label{eq:series-X1-X2-assymetry}
\begin{split}
    X_{1,n} &\doteq \cos(\lambda_0 n) Y_{1,n} + \sin(\lambda_0 n) Y_{2,n}, \quad n \in \ZZ, \\
    X_{2,n} &\doteq \cos(\lambda_0 n) \tilde Y_{1,n} + \sin(\lambda_0 n) \tilde Y_{2,n}, \quad n \in \ZZ,
\end{split}
\end{equation}
then $c_{1,f}^+, c_{2,f}^- > 0$ and $c_{1,f}^-, c_{2,f}^+ = 0$, where $c_{i,f}^+$ (resp $c_{i,f}^-$), $i=1,2$, is the coefficient of $X_i = \{X_{i,n}\}_{n \in \ZZ}$ in the spectral domain as $\lambda \to \lambda_0^+$ (resp. $\lambda \to \lambda_0^-$). We remark that, from the calculations in Section \ref{appendix:acvf-spec-clm} of the Appendix, $c_{1,f}^- = 0$ implies the critical case $\phi_1 = \pi \left(  \frac{1}{2} -d_1 \right)$, where, as $h \to \infty$,
\[
\gamma_{X_1} (h) \sim \cos( \lambda_0 h + \phi_1) h^{2d_1-1} = \cos \left( \lambda_0 h - \pi d_1 + \frac{\pi}{2}\right) h^{2d_1-1}  = \sin( \pi d_1 - \lambda_0 h) h^{2d_1-1}, 
\]
and so 
\[
c_{1,f}^+ = \frac{c_\gamma}{2\pi} \Gamma(2d_1) \cos(d_1\pi - \phi_1) = \frac{c_\gamma}{2\pi} \Gamma(2d_1) \cos\left(2 d_1\pi - \frac{\pi}{2}\right) = \frac{c_\gamma}{2\pi} \Gamma(2d_1) \sin\left(2 d_1\pi \right).
\]
Analogous calculations show that $c_{2,f}^+ = 0$ implies that, with $\phi_2$ the cyclical phase parameter of $X_2$,  $\phi_2 = \pi \left( d_2 - \frac{1}{2}   \right)$, and so, as $h \to \infty$,
\[
\gamma_{X_2} (h) \sim \sin( \pi d_2 + \lambda_0 h) h^{2d_2-1}, \quad c_{2,f}^- = \frac{c_\gamma}{2\pi} \Gamma(2d_2) \sin(2 d_2 \pi )
\]
Now consider the sum
\begin{equation} \label{eq:series-assym-memory}
X_n \doteq X_{1,n} + X_{2,n} = \cos(\lambda_0 n) ( Y_{1,n} + \tilde Y_{1,n}) + \sin(\lambda_0 n) ( Y_{2,n} + \tilde Y_{2,n}), \quad n \in \ZZ.
\end{equation}
Since $X_1,X_2$ are independent, it is clear to see that the series defined by \eqref{eq:series-assym-memory}-\eqref{eq:series-X1-X2-assymetry} satisfies \eqref{eq:cyclical-spectrum-assymetry-memory}, with
\begin{align}
 f_X(\lambda) &\sim 
 \begin{cases}
       c_{1,f}^+ (\lambda - \lambda_0)^{-2d_1}, &\quad\text{as}\; \lambda \to \lambda_0^+\\
       c_{2,f}^- (\lambda_0 - \lambda)^{-2d_2}, &\quad\text{as}\; \lambda \to \lambda_0^-
 \end{cases}, \label{eq:assym-spectral}\\
 \gamma_X(h) &\sim h^{2d_1 -1} \sin(\pi d_1 - \lambda_0 h) + h^{2d_2 -1} \sin(\pi d_2 + \lambda_0 h), \quad \text{as } h \to \infty. \label{eq:assym-ACVF}
\end{align}

The only CLM model we are aware of exhibiting a cyclical phase $\phi \neq 0$ is the Seasonal Cyclical Asymetric Long Memory (CSALM) of \cite{Arteche20003}. It is curious that the general CSALM model constructed there (see, e.g., (2.3),(2.4),(2.5) of the same paper) exhibits the same cyclical phase in the asymptotics of the ACVF as in \eqref{eq:assym-ACVF}. \PZ{Was it expected?}

\textbfWe now extend our argument to the case of a $k$-factor CLM process, for which two non-equivalent characterizations have been used in the literature. In the time domain, we will say that a time series exhibits \textit{cyclical long memory with $k-$factors} ($k-$CLM for short) if
\begin{equation} \label{eq:k-clm-acvf}
    \gamma_X(h) \sim \sum_{i=1}^k c_i \cos(\lambda_i h + \phi_i) h^{2d_i-1}, \quad \text{as} \; h \to \infty,
\end{equation}
where $d_i \in (0,1/2), \phi_i \in \cli_{d_i}$, with $\cli_{d_i}$ the set of admissible cyclical phases presented in \eqref{eq:admissible-set}, and $\lambda_i \in (0,\pi)$ for $i = 1,\dots,k$. In the literature (to the best of our knowledge), only models with $\phi_i = 0$ for all $i$ have been considered. In the spectral domain, we can think of series exhibiting $k-$CLM as having the following approximate density for all $i=1,\dots,k$
\begin{equation} 
 f_X(\lambda - \lambda_i) \sim 
 \begin{cases}
       c_{f,i}^+ (\lambda)^{-2d} &\quad\text{as}\; \lambda \to 0^+\\
       c_{f,i}^- (- \lambda)^{-2d} &\quad\text{as}\; \lambda \to 0^-
 \end{cases},
\end{equation}
for some constants $\{ c_{f,i}^+\}_{i=1}^k,\{ c_{f,i}^-\}_{i=1}^k$. As in the standard CLM case, we are not aware of a rigorous argument relating these two characterizations, and this will be addressed in a future work.

It turns out that it is possible to construct a model exhibiting $k-$CLM by means of $k$ bivariate time series $\{Y_{i,n}\}_{n \in \ZZ}$ with $i = 1,\dots,k$ as follows. Let for fixed $i =1,\dots,k$, $\{Y_{i,n}\}_{n \in \ZZ}, $ be a bivariate VARFIMA$(0,D_i,0)$ model with $D_i = \diag(d_i,d_i)$. Let, in addition, $Y_{i,n}$ and 
$Y_{j,n}$ be independent if $i\neq j$, and
\begin{equation} \label{eq:Yin-multiple}
Y_{i,n} = (I-B)^{-D_i} Q_{+,i} \veps_{n,i} + (I-B^{-1})^{-D_i} Q_{-,i} \veps_{n,i}, \quad i=1,\dots,k
\end{equation}
where $\{\veps_{n,i}\}_{n \in \ZZ}$ are bivariate WN sequences with $\EE \veps_{n,i} = 0$, $\EE \veps^T_{n,i} \veps_{n,i} = I$, and for each $i$, $Q_{-,i}, Q_{+,i}$ are matrices of the form \eqref{eq:def-Q+-} leading to a cyclical phase of $\phi_i$ respectively. We denote their respective ACVF by $\gamma^{Y,i}$. In particular, $Y_{i,n}, i = 1,\dots,k$ satisfy Property \eqref{Property1} by an application of Theorem \ref{thm:Yn-constr}. Let
\begin{equation} \label{eq:cycl-mult-spectra-phase}
    X_n = \sum_{i=1}^k \left[  \cos(\lambda_i n) Y_{i,n}^{(1)} + \sin(\lambda_i n) Y_{i,n}^{(2)} \right].
\end{equation}

\begin{proposition}
    Let, for all $i=1,\dots,k$, $\{Y_{i,n}\}_{n \in \ZZ}$ be stationary, bivariate LM series given \eqref{eq:Yin-multiple} where $Q_{+,i},Q_{-,i}$ is as in \eqref{eq:def-Q+-}, with $q_0$ replaced by $q_{0,i}$ and $q_1$ by $q_{1,i}$. Let, moreover, $\{X_n\}_{n \in \ZZ}$ be given by \eqref{eq:cycl-mult-spectra-phase} for some constants $\lambda_1,\dots,\lambda_k \in (0,\pi)$. Then, $\{X_n\}_{n \in \ZZ}$ is stationary. Additionally, the series exhibit $k-$CLM, i.e. admit the ACVF in \eqref{eq:k-clm-acvf} for these values of $\lambda_1,\dots,\lambda_k$ and
    \begin{equation} \label{eq:phi-def-multi}
    \phi_i \doteq \arccos \left(\frac{a_i}{\sqrt{a_i^2 + b_i^2}}\right),
\end{equation}
where
 \begin{equation} \label{eq:def-ai-bi}
     a_i \doteq \frac{1}{\Gamma(2d)} \left[ q_{0,i}^2 \left( 2 \frac{\sin(\pi d)}{\sin(2 \pi d)} + 1  \right) + q_{1,i}^2 \left( 2 \frac{\sin(\pi d)}{\sin(2 \pi d)} - 1  \right) \right] , \quad b_i \doteq \frac{q_{0,i} q_{1,i}}{\Gamma(2d)}.
    \end{equation}
\end{proposition}

% \begin{proposition}
% Let $\{X_n\}_{n \in \ZZ}$ be given by \eqref{eq:cycl-mult-spectra-phase}, with $\{Y_{i,n}\}_{n \in \NN_0}$ defined in \eqref{eq:Yin-multiple} and $Q_{+,i},Q_{-,i}$ of the form \eqref{eq:def-Q+-} for some families $\{q_{0,i}\}_{i =1}^k$, $\{q_{1,i}\}_{i=1}^k$. Then, $X_n$ exhibits $k-$CLM with singularities in the spectral frequency at $\lambda_1,\dots,\lambda_k$ and cyclical phase parameters $\phi_1,\dots,\phi_k$ obtained by $Q_{+,i},Q_{-,i}$ (see Remark \ref{rmk:phi-q0q1}). In particular, $X_n$ is second-order stationary.
% \end{proposition}

\begin{proof}
The proof is analogous to Proposition \ref{thm:constr}. We include it here for completeness. Fix $h,n \in \NN_0$, then
\begin{equation} \label{eq:X-ACVF-mult-1}
\begin{split}
    \EE X_{n+h} X_n^T  &= \sum_{i=1}^k \left[\cos(\lambda_i n) \cos( \lambda_i (n+h)) \gamma^{Y,i}_{11}(h) + \sin(\lambda_i n) \sin( \lambda_i (n+h)) \gamma^{Y,i}_{22}(h) \right. \\
    &+ \left. \cos(\lambda_i n) \sin( \lambda_i (n+h)) \gamma^{Y,i}_{12}(h) + \sin(\lambda_i n) \cos( \lambda_i (n+h)) \gamma^{Y,i}_{21}(h)\right], 
\end{split}
\end{equation}
Define $\phi_i$ by \eqref{eq:phi-def-multi} and recall that, from \eqref{Property1}, we have  $\gamma_{11}^{Y,i}(h) = \gamma_{22}^{Y,i}(h)$ and $\gamma_{12}^{Y,i}(h) = - \gamma_{21}^{Y,i}(h)$ for all $i = 1,\dots,k$. 
This, together with the last two displays and Property \eqref{eq:R-Y} imply that
% Since $d_1 = d_2 = d$, we have that 
% \[
% \gamma_X(n) = (R_{jk}(n) n^{d_j+d_k -1})_{j,k=1,2} = (R_{jk}(n) n^{2d-1})_{j,k=1,2},
% \]
% where 
% \[
% R \doteq
% \begin{pmatrix}
% c_1 & c_2 \\
% -c_2 & c_1 
% \end{pmatrix}
% \]
% for some constancts $c_1,c_2$ to be determined. 
\begin{equation} \label{eq:acvf-X-Y-multip}
\begin{split}
    \gamma_X(h) &=  \sum_{i=1}^k \bigg[ \gamma_{11}^{Y,i}(h) \left( \cos(\lambda_i n) \cos( \lambda_i (n+h)) + \sin(\lambda_i n) \sin( \lambda_i (n+h))   \right) \bigg. \\
    &+ \bigg. \gamma_{12}^{Y,i}(h) \left(\cos(\lambda_i n) \sin( \lambda_i (n+h)) - \sin(\lambda_i n) \cos( \lambda_i (n+h)) \right) \bigg] \\
    &= \sum_{i=1}^k \gamma^{Y,i}_{11}(h) \cos(\lambda_i h) + \gamma^{Y,i}_{12}(h) \sin(\lambda_i h) \\
    &= \sum_{i=1}^k \sqrt{(a_i^2 + b_i^2)} \left[ \frac{a_i}{\sqrt{(a_i^2 + b_i^2)}} \cos(\lambda_i h) - \frac{b_i}{\sqrt{(a_i^2 + b_i^2)}} \sin(\lambda_i h)       \right]h^{2d-1} \\
&= \sum_{i=1}^k \sqrt{(a_i^2 + b_i^2)} \left[ \cos(\phi_i) \cos(\lambda_i h) - \sin(\phi_i) \sin(\lambda_i h)       \right]h^{2d-1} \\
    &= \sum_{i=1}^k \sqrt{(a_i^2 + b_i^2)} \cos(\lambda_0 h + \phi_i) h^{2d-1}.
\end{split}
\end{equation}
 This says that $\gamma_X(h)$ does not depend on $n$, and so $X$ is stationary. Additionally, it says that $\{X_n\}_{n \in \NN_0}$ admits the ACVF of \eqref{eq:k-clm-acvf} and thus exhibits $k$-CLM. The display in \eqref{eq:def-ai-bi} is merely an application of Theorem \ref{thm:Yn-constr} for each $\{Y_{i,n}\}_{n \in \ZZ}, i = 1,\dots,k$. 
\end{proof}

\begin{remark}
    A more general result can be obtained by replacing the VARFIMA$(0,D_i,0)$ bivariate series that have been used as building blocks by general linear series (see Theorem \ref{thm:linear-repr-biv}). In this case, the fourth line of \eqref{eq:acvf-X-Y-multip} only holds asymptotically as $h \to \infty$.
\end{remark}

\begin{remark}
    Instead of considering $k$ bivariate time-series satisfying \eqref{Property1} 
 and \eqref{eq:ACVF-Y} with respective $R_i$, one can also choose a $2k-$variate time-series satisfying 
 \[
 \gamma^{Y}_{(2i-1)(2i-1)}(h) =  \gamma^{Y}_{(2i)(2i)}(h), \quad \gamma^{Y}_{(2i-1)(2i)}(h) =  -\gamma^{Y}_{(2i)(2i-1)}(h), \quad  \text{for all}\; h \in \ZZ \; \text{and}\; i=1,\dots,k.
 \]
with asymptotic ACVF including the block-diagonal matrix
    \[
    R(h) \doteq \begin{bmatrix}
    R_1   &   0       & 0         & \cdots    & 0\\
0 &   R_2       & 0         & \cdots    & 0\\
0 & 0   &  R_3         & \cdots    & 0\\
\vdots  & \vdots    & \vdots    & \ddots    & \vdots\\
0 & 0  & \cdots  & 0 & R_k
  \end{bmatrix},
    \quad
    R_i = \begin{pmatrix}
        a_i & -b_i \\
        b_i & a_i
    \end{pmatrix}, \quad i = 1,\dots, k.
    \]
\end{remark}



In fact it is also possible to obtain the standard $k-$CLM considered in the literature, where $\phi_i = 0$ for $i=1,\dots,k$. 
Let $\{Y_{i,n}\}_{n \in \ZZ}$, $i= 1,\dots,2k$ be independent univariate LM time-series with ACVF given by $\gamma_{j,Y}(h) = \EE Y_{2j-1,n} Y_{2j-1,n+h} = \EE Y_{2j,n} Y_{2j,n+h} \sim c_j h^{2d_j-1}$ as $h \to \infty$, for $j=1,\dots,k$. Define 
\begin{equation} \label{eq:cycl-mult-spectra}
    X_n = \sum_{i=1}^k \left[  \cos(\lambda_i n) Y_{2i-1,n} + \sin(\lambda_i n) Y_{2i,n} \right]
\end{equation}
Then, we have the following trivial corollary, whose proof we ommit.

\begin{corollary}
    Define $\{X_n\}_{n \in \NN_0}$ as in \eqref{eq:cycl-mult-spectra} for some $\lambda_1,\dots,\lambda_k \in (0,\pi)$, where $\{Y_{i,n}\}_{n \in \ZZ}, i = 1,\dots,2k$ are constructed as above the equation. Then, $X_n$ is stationary $k-$CLM with $\phi_i = 0$ and the same $\lambda_i$ used in the construction for all $i=1,\dots,k$.
\end{corollary}


% \PZ{
% \subsection{Two Sided Linear Representations for Cyclical Long Memory Model}

% In this Section, we investigate the linear representation of the constructed CLM series constructed from a VARFIMA$(0,D,0)$ model. Recall that $Y_n$ admits the bivariate representation
% \[
% Y_n = (I - B)^{-D} Q_+ \veps_n + (I - B^{-1})^{-D} Q_- \veps_n,
% \]
% where $Q_-,Q_+$ are defined in \eqref{eq:def-Q+-} and $\veps_n = (\xi_n,\eta_n) \in \RR^2$ is a bivariate white noise. Let the following operators admit the formal series expansions
% \[
% (I- B)^{-d} = \sum_{k=0}^\infty a_k B^k, \quad (I- B^{-1})^{-d} = \sum_{k=0}^\infty a_k B^{-k},
% \]
% for some appropriate sequence $\{a_k\}_{n \in \NN_0}$. Then, we obtain 
% \[
% Y_n^{(1)} = q_0 \sum_{k \in \NN} a_k \xi_{n-k} + q_0 \sum_{k \in \NN} a_k \xi_{n+k} + q_1 \sum_{k \in \NN} a_k \eta_{n-k} - q_1 \sum_{k \in \NN} a_k \eta_{n+k},
% \]
% and
% \[
% Y_n^{(2)} = - q_1 \sum_{k \in \NN} a_k \xi_{n-k} + q_1 \sum_{k \in \NN} a_k \xi_{n+k} + q_0 \sum_{k \in \NN} a_k \eta_{n-k} + q_0 \sum_{k \in \NN} a_k \eta_{n+k}.
% \]
% This says that 
% \begin{equation}
% \begin{split}
%     X_n &= \cos(\lambda_0 n ) Y_n^{(1)} + \sin(\lambda_0 n) Y_n^{(2)} \\
%     &= \left[ \cos(\lambda_0 n ) q_0 -  \sin(\lambda_0 n) q_1    \right] \sum_{k \in \NN} a_k\xi_{n-k} + \left[ \cos(\lambda_0 n ) q_0 +  \sin(\lambda_0 n) q_1    \right] \sum_{k \in \NN} a_k \xi_{n+k} \\
%     &+\left[  \cos(\lambda_0 n ) q_1 +  \sin(\lambda_0 n) q_0    \right] \sum_{k \in \NN} a_k \eta_{n-k} +\left[  - \cos(\lambda_0 n ) q_1 +  \sin(\lambda_0 n) q_0    \right] \sum_{k \in \NN} a_k \eta_{n+k} \\
%     &= c \left[ \cos(\lambda_0 n + \psi )  \sum_{k \in \NN} a_k \xi_{n-k} +  \cos(\lambda_0 n - \psi )  \sum_{k \in \NN} a_k \xi_{n+k} + \sin(\lambda_0 n + \psi)  \sum_{k \in \NN} a_k \eta_{n-k} + \sin(\lambda_0 n - \psi)  \sum_{k \in \NN} a_k \eta_{n+k} \right],
% \end{split}
% \end{equation}
% where $\psi \doteq \arccos \left( \frac{q_0}{\sqrt{q_0^2 + q_1^2}} \right)$ and $c \doteq \sqrt{q_0^2 + q_1^2}$. This says that by defining
% \[ 
% \tilde a_{k,n} \doteq \begin{cases} 
%       c \cos(\lambda_0 n  - \psi) a_k  & k \ge 1 \\
%       2 c a_k \cos(\lambda_0 n) \cos(\psi) & k = 0 \\
%       c \cos(\lambda_0 n + \psi) )a_j & k \le -1 
%    \end{cases}, \quad  
% \tilde b_{k,n} \doteq \begin{cases} 
%       c \sin(\lambda_0 n  - \psi) a_k  & k \ge 1 \\
%       2 c a_k \sin(\lambda_0 n) \cos(\psi) & k = 0 \\
%       c \sin(\lambda_0 n + \psi) )a_j & k \le -1 
%    \end{cases} ,
% \]
% we can see that $X_n$ can be written as the sum of two double-sided series
% \[
% X_n = \sum_{k \in \ZZ} \tilde a_{k,n} \xi_{n+k} + \sum_{k \in \ZZ} \tilde b_{k,n} \eta_{n+k}
% \]
% We remark that this representation is not the usual linear representation since the coefficients of the noise depend on the time $n$ of the time series $X_n$.
% }

\newpage

Under somewhat strict conditions on $L$ we have that as $\theta \to 0^+$,
\[
\sum_{n=1}^\infty L(n) \frac{\sin(n \theta)}{n^{\alpha}} \sim \frac{L(1/\theta)}{\theta^{1-\alpha}} \frac{\frac{1}{2}\pi}{\Gamma(\alpha)\sin(\frac{1}{2}\pi \alpha)}
\]
(see \cite{bingham_goldie_teugels_1987}, below equation (6.1) and also on the section for Abel summability for conditions on $L$). Allegedly this holds for $-1 < \alpha \le 0$ as well (under the stricter conditions), but this display doesn't make sense for the desired value $\alpha = 0$.

\newpage

Finally take $- \frac{1}{2} < \delta < 0$. Clearly,
\[
|\int_0^{\lambda_0} \cos(h \lambda ) L_{f,1}\left( \frac{1}{\om} \right) \om^{-2\delta} d\om | \le \int_0^{\lambda_0} |L_{f,1}\left( \frac{1}{\om} \right) \om^{-2\delta}| d\om    = O(1),
\]
and the same asymptotics holds for the sine Fourier coefficient, which says that
\begin{equation}
\begin{split}
\gamma_-(h) &= \cos(h \lambda_0) \int_0^{\lambda_0} \cos(h \lambda ) L_{f,1}\left( \frac{1}{\om} \right) \om^{-2\delta} d\om + \sin(h \lambda_0) \int_0^{\lambda_0} \sin(h \om )  L_{f,1}\left( \frac{1}{\om} \right) \om^{-2\delta} d\om  \\
    &= O(1).
\end{split}
\end{equation}

\newpage

\begin{proposition} \label{it:spec-to-time-border} 
    Let 
    \[
    c_f^- = 0, \quad R_f^\pm(x) = L_f^\pm \left( \frac{1}{x}  \right) x^{-2\veps_{\pm}}, 
    \]
    where $L_f^-: \left(\frac{1}{\lambda_0},\infty\right) \to (0,\infty)$, $L_f^+: \left(\frac{1}{\pi - \lambda_0},\infty\right) \to (0,\infty)$ are two quasi-monotone slowly varying functions at $+\infty$, with $L_f^\pm(x) \sim b_f^\pm \in (0,\infty)$ as $x \to \infty$, and $\veps_\pm \in (0,d)$. Then, Definition \ref{defn:clm-spec} implies Definition \ref{defn:clm-time} in the ``boundary" case with
    \begin{equation} \label{eq:cgamma-phi-boundary}
        c_\gamma \doteq 2\Gamma(1-2d) c_f^+, \quad \phi \doteq \left( \frac{1}{2} - d \right) \pi,
    \end{equation}
    and
    \begin{equation} \label{eq:rgamma-boundary}
    \begin{split}
        R_\gamma(h) &\doteq  2 \Gamma(1-2d + 2\veps_+) L_{f}^+\left(h \right) \left(  \sin((d - \veps_+) \pi)   \cos(\lambda_0 h) - \cos((d - \veps_+) \pi)   \sin(\lambda_0 h) \right) h^{- 2\veps_+} \\
    &\quad+ 2\Gamma(1-2d + 2\veps_-) L_{f}^-(h) \left( \sin((d - \veps_- ) \pi ) \cos(h \lambda_0) + \cos((d - \veps_- ) \pi ) \sin(h \lambda_0 ) \right) h^{-2 \veps_-}
     \\
    &\quad   + o(h^{- 2\veps_+}) + (\cos(\lambda_0 h) + \sin(\lambda_0 h) )O(h^{-2d}).
    \end{split}
    \end{equation}
\end{proposition}


\begin{proof}
Recall the display in \eqref{eq:210}. In view of \eqref{eq:spec-to-time-gamma+} and the form of $R_f^+$ in the assumption, we write
\begin{equation} \label{eq:bound-g+}
\begin{split}
   2\gamma_+(h) &= 2\cos(h \lambda_0) \int_0^{\pi - \lambda_0} \cos(h  \om ) R_{f}^+\left(\om\right) \om^{-2d} d\om - 2\sin(h \lambda_0) \int_0^{\pi - \lambda_0} \sin(h  \om ) R_{f}^+\left(\om\right) \om^{-2d} d\om \\
   &= 2 c_f^+ \cos(h \lambda_0) \int_0^{\pi - \lambda_0} \cos(h  \om ) \om^{-2d } d\om - 2 c_f^+ \sin(h \lambda_0) \int_0^{\pi - \lambda_0} \sin(h  \om )  \om^{-2d} d\om \\
   &\quad + 2 \cos(h \lambda_0) \int_0^{\pi - \lambda_0} \cos(h  \om )  L_{f}^+\left(\frac{1}{\om}\right) \om^{-2d + 2\veps_+} d\om \\
   &\quad- 2\sin(h \lambda_0) \int_0^{\pi - \lambda_0} \sin(h  \om )  L_{f}^+\left(\frac{1}{\om}\right) \om^{-2d +2 \veps_+} d\om \\
   &= c_\gamma \cos(\lambda_0 h + \phi) h^{2d-1} \\
   &\quad+ 2 \Gamma(1-2d + 2\veps_+) \sin((d - \veps_+) \pi)  L_{f}^+\left(h \right) \cos(\lambda_0 h) h^{2d-1 - 2\veps_+} \\
   &\quad-  2 \Gamma(1-2d + 2\veps_+) \cos((d - \veps_+) \pi)  L_{f}^+\left(h \right) \sin(\lambda_0 h) h^{2d-1 - 2\veps_+} + o(h^{2d-1 - 2\veps_+}) 
\end{split}
\end{equation}
where the third equality follows from Lemma \ref{lemma-second-order-spec-to-time} and Proposition A.2.2 of \cite{pipiras_taqqu_2017} since $-2d +2 \veps_+ < 0$, and $\phi,c_\gamma$ were defined in \eqref{eq:cgamma-phi-boundary}.

Now we compute the contribution of $\gamma_-$. From Proposition A.2.2 of \cite{pipiras_taqqu_2017} and the form of $R_f^-$, as $h \to \infty$
\begin{equation} \label{eq:bound-g-}
\begin{split}
2\gamma_-(h) &= 2\cos(h \lambda_0) \int_0^{\lambda_0} \cos(h \lambda ) R_{f}^-\left( \om \right) \om^{-2 d} d\om + 2\sin(h \lambda_0) \int_0^{\lambda_0} \sin(h \om )  R_{f}^-\left( \om \right) \om^{-2d} d\om  \\
&= 2\cos(h \lambda_0) \int_0^{\lambda_0} \cos(h \lambda ) L_{f}^-\left( \frac{1}{\om} \right) \om^{-2 d + 2\veps_- } d\om + 2\sin(h \lambda_0) \int_0^{\lambda_0} \sin(h \om )  L_{f}^-\left( \frac{1}{\om} \right) \om^{-2d + 2\veps_-} d\om \\
    &\sim 2\Gamma(1-2d + 2\veps_-) L_{f}^-(h) \left(\cos(\pi (d - \veps_- )) \sin(h \lambda_0 )+ \sin(\pi (d - \veps_- )) \cos(h \lambda_0) \right) h^{2d-1 - 2\veps_-}.
\end{split}
\end{equation}
Combining \eqref{eq:210}, \eqref{eq:bound-g+}, and \eqref{eq:bound-g-}, we write
\begin{equation}
\begin{split}
    \gamma_X(h) &= 2 \gamma_{+}(h) + 2 \gamma_-(h) \\
    &= c_\gamma \cos(\lambda_0 h + \phi) h^{2d-1} \\
    &\quad+ 2 \Gamma(1-2d + 2\veps_+) \sin((d - \veps_+) \pi)  L_{f}^+\left(h \right) \cos(\lambda_0 h) h^{2d-1 -2 \veps_+} \\
   &\quad-  2 \Gamma(1-2d + 2\veps_+) \cos((d - \veps_+) \pi)  L_{f}^+\left(h \right) \sin(\lambda_0 h) h^{2d-1 - 2\veps_+} \\
    &\quad+ 2\Gamma(1-2d + 2\veps_-) L_{f}^-(h) \left(\cos(\pi (d - \veps_- )) \sin(h \lambda_0 )+ \sin(\pi (d - \veps_- )) \cos(h \lambda_0) \right) h^{2d-1 -2 \veps_-}
     \\
    &\quad   + o(h^{2d-1 - 2\veps_+}) + (\cos(\lambda_0 h) + \sin(\lambda_0 h) )O(h^{-1}) \\
    &=   c_\gamma \cos(\lambda_0 h + \phi) h^{2d-1} + R_\gamma(h) h^{2d-1}, 
\end{split}
\end{equation}
where $c_\gamma,\phi$ and $R_\gamma$ were defined in \eqref{eq:cgamma-phi-boundary}--\eqref{eq:rgamma-boundary}. 
\end{proof}

\begin{remark}
    Note that, as $h \to \infty$, the leading term of $R_\gamma$ in \eqref{eq:rgamma-boundary} is given by 
    \begin{equation}
        R_\gamma(h) \sim \begin{cases}
        2 \Gamma(1-2d + 2\veps_+) b_f^+\left(  \sin((d - \veps_+) \pi)   \cos(\lambda_0 h) - \cos((d - \veps_+) \pi)   \sin(\lambda_0 h) \right) h^{- 2\veps_+} & \veps_+ < \veps_-, \\
        \begin{aligned} 
        &2 \Gamma(1-2d + 2\veps) (b_f^- + b_f^+ )  \sin((d - \veps) \pi)   \cos(\lambda_0 h) h^{- 2\veps} \\ 
        &+ 2 \Gamma(1-2d + 2\veps) (b_f^- - b_f^+ )  \cos((d - \veps) \pi)   \sin(\lambda_0 h)  h^{- 2\veps} \end{aligned} & \veps_+ = \veps_- = \veps,   \\
    2\Gamma(1-2d + 2\veps_-) b_{f}^- \left( \sin((d - \veps_- ) \pi ) \cos(h \lambda_0) + \cos((d - \veps_- ) \pi ) \sin(h \lambda_0 ) \right) h^{- 2\veps_-} & \veps_+ > \veps_-.
        \end{cases}
    \end{equation}
\end{remark}

When going from the time to the spectral domain, the term $c_\gamma \cos(\lambda_0 h + \phi) h^{2d-1}$ in Definition \ref{defn:clm-time} will lead to $c_f^- (\lambda_0 - \lambda)^{-2d}$, $c_f^+ (\lambda - \lambda_0)^{-2d}$ in Definition \ref{defn:clm-time}, plus a remainder of the order $o(|\lambda - \lambda_0|^{-2d})$. The ultimate remainders $R_f^\pm$ in Definition \ref{defn:clm-time} will be determined by the exact form of $R_\gamma(h)$.


In Appendix \ref{app:subsec-time-to-spec-non-boundary} we state and prove a result in the ``non-boundary" case $\phi \in \left( -\left( \frac{1}{2} -d \right) \pi, \left( \frac{1}{2} -d \right) \pi \right)$. A special treatment is required for the ``boundary" case $\phi = \pm \left( \frac{1}{2} -d \right) \pi$, and state a related result in Appendix \ref{app:subsec-time-to-spec-boundary}. Recall the sign function in \eqref{def:sign-func}.

\subsection{``Non-boundary" case} \label{app:subsec-time-to-spec-non-boundary}

\begin{proposition} \label{prop:equiv-defn-time-to-spec} 
    Assume that $\phi \in \left(\left(d - \frac{1}{2} \right)\pi  , \left(\frac{1}{2} - d\right) \pi \right)$, and that for $h \ge 1$,
    \begin{equation} \label{eq:time-to-spec-rgamma}
        R_\gamma(h) \doteq (L_{1,\gamma}(h) - c_{\gamma} \cos(\phi)) \cos(\lambda_0 h)  + \operatorname{sign}(-\sin(\phi)) (L_{2,\gamma}(h) - |c_{\gamma} \sin(\phi) |) \sin(\lambda_0 h) ,
    \end{equation}
    where $L_{1,\gamma}, L_{2,\gamma} : (0,\infty) \to (0,\infty)$ are slowly varying functions at $+\infty$, quasi-monotone, with $L_{1,\gamma}(x) \sim c_{\gamma} \cos(\phi) \in (0,\infty)$ and $L_{2,\gamma}(x) \sim |c_{\gamma} \sin(\phi) | \in [0,\infty)$ as $x \to \infty$.  Then, Definition \ref{defn:clm-time} implies Definition \ref{defn:clm-spec} with 
    % $L_f^+(x)  \sim c_f^+$ and $L_f^-(x)  \sim c_f^-$ as $x \to + \infty$, where
        \begin{equation} \label{eq:cfpm-cgamma}
    c_f^\pm \doteq \frac{c_\gamma}{2\pi} \Gamma(2d) \cos(\pi d \mp \phi),
\end{equation}
and
\begin{equation} \label{eq:rf+-phi-cg}
\begin{split}
    R_f^\pm(\lambda) &\doteq \frac{\Gamma(2d)}{2\pi} \left[ \left( L_{1,\gamma} \left(  \frac{1}{|\lambda - \lambda_0|}  \right) - c_\gamma \cos(\phi)  \right)\cos(d\pi) \right. \\
    &\quad \left. \mp \left(  \operatorname{sign}(-\sin(\phi)) L_{2,\gamma} \left(  \frac{1}{|\lambda - \lambda_0|}  \right) + c_\gamma \sin(\phi) \right) \sin(d\pi)   \right] + o(1).
\end{split}
\end{equation}
\end{proposition}


\begin{proof}
As in the proof of Proposition 2.2.14 in the Appendix of \cite{pipiras_taqqu_2017}, for $\lambda \in [0,\pi) \setminus \{\lambda_0\}$,
\begin{equation}
f_X(\lambda) =  \frac{1}{2\pi} \sum_{h=-\infty}^{\infty} e^{-ih\lambda} \gamma_X(h).
\end{equation}
Strictly speaking, the arguments below are first used to show that the spectral density can be written this way and then the asymptotics are established. In particular,
\begin{equation} \label{eq:456}
\begin{split}
        f_X(\lambda) &=  \frac{1}{2\pi} \left[ \gamma_X(0) + 2\sum_{h=1}^\infty \cos( h \lambda ) \left(L_{1,\gamma}(h) \cos( \lambda_0 h ) + \operatorname{sign}(-\sin(\phi))  L_{2,\gamma}(h) \sin( \lambda_0 h ) \right) h^{2d-1} \right] \\ 
    &= \frac{1}{2\pi} \left[ \gamma_X(0) + f_1(\lambda) - \operatorname{sign}(-\sin(\phi))  f_2(\lambda) +  f_3(\lambda) + \operatorname{sign}(-\sin(\phi)) f_4(\lambda) \right],
\end{split}
\end{equation}
where
\begin{equation} \label{eq:f1-f2-def}
    f_1(\lambda) \doteq \sum_{h=1}^\infty \cos\big((\lambda-\lambda_0) h \big) L_{1,\gamma}(h) h^{2d-1}, \quad f_2(\lambda) \doteq \sum_{h=1}^\infty \sin\big((\lambda-\lambda_0) h \big) L_{2,\gamma(h)} h^{2d-1},
\end{equation}
\begin{equation} \label{eq:f3-f4-def}
    f_3(\lambda) \doteq  \sum_{h=1}^\infty \cos((\lambda + \lambda_0)h  )  L_{1,\gamma}(h)  h^{2d-1}, \quad f_4(\lambda) \doteq  \sum_{h=1}^\infty \sin((\lambda + \lambda_0)h  )  L_{2,\gamma}(h)  h^{2d-1}.
\end{equation}
By Proposition A.2.1 of \cite{pipiras_taqqu_2017}, as $\lambda \to \lambda_0$,
\begin{equation} \label{eq:f1-f2}
\begin{split}
    f_1(\lambda) &= |\lambda-\lambda_0|^{-2d} L_{1,\gamma} \left(  \frac{1}{|\lambda - \lambda_0|}  \right) \Gamma(2d) \cos(\pi d) + o(|\lambda-\lambda_0|^{-2d}), \\
    f_2(\lambda) &= \text{sign}(\lambda - \lambda_0) |\lambda-\lambda_0|^{-2d} L_{2,\gamma} \left(  \frac{1}{|\lambda - \lambda_0|}  \right) \Gamma(2d) \sin(\pi d)+ o(|\lambda-\lambda_0|^{-2d}).
\end{split}
\end{equation}

% On the other hand, by using Lagrange's trigonometric identities, for each $N \in \NN$
% \[
% \sum_{h=1}^N \cos((\lambda + \lambda_0)h  ) \le \frac{1}{2} + \frac{1}{2 \min\{ \sin\left(\frac{\lambda_0}{2}\right) ,\sin\left(\frac{\pi + \lambda_0}{2}\right)  \}}, \quad \sum_{h=1}^N \sin((\lambda + \lambda_0)h  ) \le \frac{1}{\min\{ \sin\left(\frac{\lambda_0}{2}\right) ,\sin\left(\frac{\pi + \lambda_0}{2}\right)  \}}.
% \]
% Note that these bounds are uniform in $\lambda$ and that $L_{1,\gamma} h^{2d-1}, L_{2,\gamma} h^{2d-1}$ are eventually decreasing, since $L_{1,\gamma}$ and $L_{2,\gamma}$ belong to the Zygmund class. Therefore, by Dirichlet's test, $f_3(\lambda) \le M, f_4(\lambda) \le M$, for some constant $M$ that does not depend on $\lambda$. 
On the other hand, fix some $0 < \alpha < \lambda_0 < \beta < \pi$, then for $\lambda \in [\alpha-\lambda_0,\beta-\lambda_0]$ we have $\lambda + \lambda_0 \in (0,\pi)$ and hence $\sup_{\hat \lambda \in [\alpha,\beta]} \{\frac{2}{\sin(\hat \lambda/2)},\frac{2}{\cos(\hat\lambda/2)}\} < \infty$. Moreover, since $L_{1,\gamma},L_{2,\gamma}$ are quasi-monotone, the display (A.2.6) in Proposition A.2.1 of \cite{pipiras_taqqu_2017} says that, for $\lambda \in [\alpha-\lambda_0,\beta-\lambda_0]$,
\[
\left| \sum_{h=n}^\infty \cos( h (\lambda + \lambda_0 )) \frac{L_{1,\gamma}(h)}{h^{1-2d}} \right| \le \frac{2}{\sup_{\hat \lambda \in [\alpha,\beta]} \{\frac{2}{\sin(\hat \lambda/2)}\}} \frac{|L_{1,\gamma}(h)|}{n^{1-2d}} (1  + O(1)),
\]
which implies that, for all $\veps > 0$, there exists some $M \ge 1$ such that
\[
\sup_{\lambda \in [\alpha-\lambda_0,\beta-\lambda_0]} \left| \sum_{h=M}^\infty \cos( h (\lambda + \lambda_0 )) \frac{L_{1,\gamma}(h)}{h^{1-2d}} \right| < \veps.
\]
Likewise, we obtain
\[
\sup_{\lambda \in [\alpha-\lambda_0,\beta-\lambda_0]} \left| \sum_{h=M}^\infty \sin( h (\lambda + \lambda_0 )) \frac{L_{2,\gamma}(h)}{h^{1-2d}} \right| < \veps.
\]
and so 
\begin{equation} \label{eq:f3-f4}
    f_3(\lambda) = O(1), \quad f_4(\lambda) = O(1).
\end{equation}
Now define
\begin{equation}
\begin{split}
    R(\lambda) &\doteq \frac{\Gamma(2d)}{2\pi} \left[ \left( L_{1,\gamma} \left(  \frac{1}{|\lambda - \lambda_0|}  \right) - c_\gamma \cos(\phi)  \right)\cos(d\pi) \right. \\
    &\quad\left.-  \text{sign}(\lambda-\lambda_0)\left(  \operatorname{sign}(-\sin(\phi)) L_{2,\gamma} \left(  \frac{1}{|\lambda - \lambda_0|}  \right) + c_\gamma \sin(\phi) \right) \sin(d\pi)   \right]  .
\end{split}
\end{equation}
Since $L_{1,\gamma}(x) \to c_\gamma \cos(\phi) ,  \operatorname{sign}(-\sin(\phi)) L_{2,\gamma}(x) \to - c_\gamma \sin(\phi)$ as $x \to \infty$, it follows that $R(\lambda) = o(1)$. By combining \eqref{eq:456}, \eqref{eq:f1-f2} and \eqref{eq:f3-f4}, we write
\begin{equation} \label{eq:time-to-spec-density}
\begin{split}
    f_X(\lambda) &= \frac{\Gamma(2d)}{2\pi} \left[ L_{1,\gamma} \left(  \frac{1}{|\lambda - \lambda_0|}  \right) \cos(d\pi) - \operatorname{sign}(-\sin(\phi))  \text{sign}(\lambda-\lambda_0) L_{2,\gamma} \left(  \frac{1}{|\lambda - \lambda_0|}  \right) \sin(d\pi)   \right]    | \lambda - \lambda_0 |^{-2d} \\
    &\quad+ \frac{\Gamma(2d)}{2\pi} \left( \gamma_X(0) +f_3(\lambda) + \operatorname{sign}(-\sin(\phi)) f_4(\lambda) \right) + o(|\lambda-\lambda_0|^{-2d}) \\ 
    &= \frac{\Gamma(2d)}{2\pi} \left[ c_\gamma \cos(\phi)    \cos(d\pi) + \text{sign}(\lambda-\lambda_0) c_{\gamma} \sin(\phi)  \sin(d\pi)   \right]    | \lambda - \lambda_0 |^{-2d} + R(\lambda) | \lambda - \lambda_0 |^{-2d} \\
    &\quad+  O(1) + o(|\lambda-\lambda_0|^{-2d}) \\ 
    &= \left( \frac{\Gamma(2d)}{2\pi} c_\gamma \cos(\pi d - \text{sign}(\lambda-\lambda_0)\phi) + R(\lambda)   + o(1) \right) 
 |\lambda - \lambda_0 |^{-2d},
    \end{split}
\end{equation}
where $c_\gamma,\phi$ were defined in \eqref{eq:cgamma-psi}. Note that \eqref{eq:time-to-spec-density} also implies \eqref{eq:rf+-phi-cg} and finishes the proof.
\end{proof}

\begin{remark}
    In view of Remark \ref{rmk:cg-c1g-c2g}, we can recast \eqref{eq:time-to-spec-rgamma} as
        \begin{equation}
        R_\gamma(h) = (L_{1,\gamma}(h) - c_{1,\gamma}) \cos(\lambda_0 h) h^{2d-1} + \operatorname{sign}(c_{2,\gamma}) (L_{2,\gamma}(h) - |c_{2,\gamma} |) \sin(\lambda_0 h) h^{2d-1},
    \end{equation}
    where $c_{1,\gamma},c_{2,\gamma}$ are given in \eqref{eq:c1g-c2g-cg}. Then, from \eqref{eq:cfpm-cgamma}, we have that
    \begin{equation} \label{eq:cf+--from-c1g-c2g}
        c_f^\pm \doteq \frac{\Gamma(2d)}{2\pi} \left( c_{1,\gamma} \cos( \pi d) \mp  c_{2,\gamma} \sin( \pi d) \right) \in (0,\infty).
    \end{equation}
\end{remark}



\subsection{``Boundary" case} \label{app:subsec-time-to-spec-boundary}

For clarity, we we shall focus on the case 
\begin{equation} 
    \phi =  \left( \frac{1}{2} -d \right) \pi,
\end{equation}
which is expected to correspond to $c_f^- = 0$ (see the discussion in Appendix \ref{subsubsec:admis-phase}). An analogous statement can be obtained in the case $\phi = - \left( \frac{1}{2} -d \right) \pi$, corresponding to $c_f^+ = 0$.

\begin{proposition} \label{prop:equiv-defn-time-to-spec-boundary} 
    Assume that $\phi = \left(\frac{1}{2} - d\right) \pi $, and that for $h \ge 1$,
    \begin{equation} \label{eq:time-to-spec-rgamma-bound}
        R_\gamma(h) \doteq L_{1,\gamma}(h)  \cos(\lambda_0 h) h^{-2\veps} + \xi L_{2,\gamma}(h)  \sin(\lambda_0 h) h^{-2\veps},
    \end{equation}
    where $\veps \in (0,d), \xi = \pm 1$, $L_{1,\gamma}, L_{2,\gamma} : (0,\infty) \to (0,\infty)$ are slowly varying functions at $+\infty$, quasi-monotone, with $L_{1,\gamma}(x) \sim b_1 \in (0,\infty)$ and $\xi L_{2,\gamma}(x) \sim b_2 \in \RR$ as $x \to \infty$ where 
    \begin{equation} \label{eq:b1-b2-cond}
        b_1 \in \RR \; \text{and}\; b_2 = 0,\quad \text{or} \quad \frac{b_1}{b_2} \in (-\tan(\pi (d-\veps)), \tan(\pi (d-\veps))). 
    \end{equation}
    hen, Definition \ref{defn:clm-time} implies Definition \ref{defn:clm-spec} with 
    % $L_f^+(x)  \sim c_f^+$ and $L_f^-(x)  \sim c_f^-$ as $x \to + \infty$, where
        \begin{equation} \label{prop:time-to-spec-bound-cf+}
    c_f^- = 0, \quad c_f^+ \doteq   \frac{c_\gamma}{2\pi} \Gamma(2d)\sin(2\pi d),
\end{equation}
and
\begin{equation} \label{eq:rf-phi-cg-bound}
\begin{split}
    R_f^\pm(\lambda) &\doteq  \frac{\Gamma(2(d-\veps))}{2\pi} \left[ L_{1,\gamma} \left( \frac{1}{|\lambda-\lambda_0|}  \right) \cos((d-\veps)\pi) \right.   \\
&\quad\mp \left. \xi L_{2,\gamma} \left( \frac{1}{|\lambda-\lambda_0|}  \right) \sin((d-\veps)\pi)  \right] |\lambda - \lambda_0|^{2\veps} + o(|\lambda - \lambda_0|^{2\veps}).
\end{split}
\end{equation}
\end{proposition}


\begin{proof}
Note that we can write, for $h \in \ZZ$,
\begin{equation}
\gamma_X(h) = c_\gamma \cos(\lambda_0 h + \phi) h^{2d-1} + L_{1,\gamma}(h) \cos(\lambda_0 h) h^{2d-2\veps-1} + \xi L_{2,\gamma}(h) \sin(\lambda_0 h)h^{2d-2\veps-1} = \gamma_1(h) + \gamma_2(h),
\end{equation}
with
\begin{equation} 
\gamma_1(h) \doteq  c_\gamma \cos(\lambda_0 h + \phi) h^{2d-1}, \quad \gamma_2(h) \doteq L_{1,\gamma}(h) \cos(\lambda_0 h) h^{2d-2\veps-1} + \xi L_{2,\gamma}(h) \sin(\lambda_0 h) h^{2d-2\veps-1}.
\end{equation}
Calculations similar to \eqref{eq:456}--\eqref{eq:time-to-spec-density} illustrate that, as $\lambda \to \lambda_0^+$, by using the fact that $\phi = \left( \frac{1}{2} - d \right) \pi$,
\begin{equation} \label{eq:time-spec-boundary-101}
\begin{split}
    \sum_{h=-\infty}^\infty e^{-ih\lambda} \gamma_{1}(h) &= \left[ \cos(\phi) \cos(\pi d) - \text{sign}(\lambda - \lambda_0) \sin(\phi) \sin(\pi d) \right]  c_\gamma \frac{1}{2\pi} |\lambda - \lambda_0|^{-2d} + O(1) \\
    &= \sin(2 d \pi)  \frac{c_\gamma}{2\pi} \Gamma(2d) |\lambda - \lambda_0|^{-2d} + O(1),
\end{split}
\end{equation}
which, since $\veps < d$, yields the formula for $c_f^+$ in \eqref{prop:time-to-spec-bound-cf+}. 
On the other hand,  as $\lambda \to \lambda_0^-$,
\begin{equation} \label{eq:time-spec-boundary-100}
\begin{split}
  \sum_{h=-\infty}^\infty e^{-ih\lambda} \gamma_{1}(h) &= \frac{1}{2\pi} \bigg[ \gamma_1(0) + \sin(d\pi) c_\gamma\sum_{h=1}^\infty \cos((\lambda - \lambda_0) h) h^{2d-1} +  \cos(d \pi) c_\gamma \sum_{h=1}^\infty \sin((\lambda_0 - \lambda) h) h^{2d-1}\bigg. \\
  &\quad+ \bigg. \sin(d\pi) c_\gamma \sum_{h=1}^\infty \cos((\lambda + \lambda_0) h) h^{2d-1} - \cos(d\pi) c_\gamma \sum_{h=1}^\infty \sin((\lambda + \lambda_0) h) h^{2d-1} \bigg]  \\
&= \frac{1}{2\pi}\left( \gamma_1(0) + \sin(d\pi) c_\gamma \sum_{h=1}^\infty \cos((\lambda + \lambda_0) h) h^{2d-1} \right.\\
&\quad- \left.   \cos(d\pi) c_\gamma \sum_{h=1}^\infty \sin((\lambda + \lambda_0) h) h^{2d-1} + O(1) \right)\\
& \doteq O(1) ,
\end{split}
\end{equation}
where we have used the form of $\phi$ and Lemma \ref{lemma:second-order-time-to-spec} to replace the two series by $O(1)$ in the second equality, and that the series in the third and fourth line are O(1) in the last equality, which follows from the same arguments as in \eqref{eq:f3-f4}. This display verifies the form of $c_f^-$ in \eqref{prop:time-to-spec-bound-cf+}.

We now investigate the spectral density corresponding to $\gamma_2$, which roughly corresponds to the form of $R_f^\pm(\lambda)$. Since $0 < \veps < d < \frac{1}{2}$ and since $b_1,b_2$ meet condition \eqref{eq:b1-b2-cond}, this spectral density is non-negative. Calculations identical to the ones of Appendix \ref{app:subsec-time-to-spec-non-boundary} show that, as $\lambda \to \lambda_0$,
\begin{equation} \label{eq:time-spec-boundary-102}
\begin{split}
 \sum_{h=-\infty}^\infty e^{-ih\lambda} \gamma_{2} (h) &= o(|\lambda - \lambda_0|^{-2(d-\veps)})+ \frac{\Gamma(2(d-\veps))}{2\pi} \left[ L_{1,\gamma} \left( \frac{1}{|\lambda-\lambda_0|}  \right) \cos((d-\veps)\pi)  \right.   \\
 &\quad- \left. \text{sign}(\lambda-\lambda_0) \xi L_{2,\gamma} \left( \frac{1}{|\lambda-\lambda_0|}  \right) \sin((d-\veps)\pi)  \right] |\lambda - \lambda_0|^{-2(d-\veps)} .
\end{split}
\end{equation}
The displays in \eqref{eq:time-spec-boundary-100}, \eqref{eq:time-spec-boundary-101}, \eqref{eq:time-spec-boundary-102} reveal that $R_f^\pm$ are given by \eqref{eq:rf-phi-cg-bound}.
\end{proof}

We present here results on higher-order behavior of the Fourier series (integrals, resp.) of power-law coefficients (functions, resp.) that were used in Appendices \ref{app:subsec-spec-to-time-boundary} and \ref{app:subsec-time-to-spec-boundary}.

\begin{lemma} \label{lemma-second-order-spec-to-time}
    Let $ d \in \left(0, \frac{1}{2} \right)$. Then, as $h \to \infty$,
    \begin{equation}
    \begin{split}
            \int_0^{1}  \cos(h  \om )  \om^{-2d} d\om &= \Gamma(1-2d) \sin(\pi d) h^{2d-1} + \sin(h) h^{-1} + O(h^{-2}), \\
            \int_0^{1} \sin(h  \om )  \om^{-2d} d\om &= \Gamma(1-2d) \cos(\pi d) h^{2d-1} - \cos(h) h^{-1} + O(h^{-2}).
    \end{split}
    \end{equation}
\end{lemma}

\begin{proof}
    We prove the equivalent identity
    \begin{equation}
        \int_0^{1}  e^{i h \om}  \om^{-2d} d\om = \Gamma(1-2d) e^{i \pi (\frac{1}{2} - d) } h^{2d-1} - i e^{ih} h^{-1} + O(h^{-2}).
    \end{equation}
    Write 
    \begin{equation} \label{eq-fourier-power-law-1}
        \int_0^{1}  e^{i h \om}  \om^{-2d} d\om = \int_0^\infty  e^{i h \om}  \om^{-2d} d\om - \int_{1}^\infty  e^{i h \om}  \om^{-2d} d\om,
    \end{equation}
    where, from formulas 3.761(4) and 3.761(9) in \cite{Graryz15} with $\mu = 1-2d, a = 1$,
    \begin{equation} \label{eq-fourier-power-law-2}
        \int_0^\infty  e^{i h \om}  \om^{-2d} d\om = h^{2d-1} \int_0^\infty e^{iz} z^{-2d} dz = \Gamma(1-2d) e^{i \pi (\frac{1}{2} - d) } h^{2d-1}.
    \end{equation}
    Moreover, 
    \begin{equation} \label{eq-fourier-power-law-3}
    \begin{split}
      \int_{1}^\infty  e^{i h \om}  \om^{-2d} d\om &= h^{2d-1} \int_h^\infty e^{iz} z^{-2d} dz \\
      &= h^{2d-1}  \int_{h}^\infty  e^{i z}  z^{-2d} dz \\
      &= h^{2d-1} \left( h^{-2d} e^{iz} i - 2d h^{-2d-1} e^{ih} + O(h^{-2d-3} )   \right) \\
      &= e^{iz} i h^{-1} + O(h^{-2}).
    \end{split}
    \end{equation}
    Combining \eqref{eq-fourier-power-law-1}, \eqref{eq-fourier-power-law-2}, and \eqref{eq-fourier-power-law-3} we obtain the desired result.
\end{proof}




\begin{lemma} \label{lemma:second-order-time-to-spec}
   For $d \in (0,1/2)$, as $\om \to 0^+$,
    \begin{equation}
    \begin{split}
       \sum_{k=1}^\infty \sin(k \om) k^{2d-1} = \om^{-2d} \Gamma(2d) \sin(\pi d) + R_1(\om), \\
       \sum_{k=1}^\infty \cos(k \om) k^{2d-1} = \om^{-2d} \Gamma(2d) \cos(\pi d) + R_2(\om),
    \end{split}
    \end{equation}
    where $R_i(\om) \to c_i \in \RR$, $i=1,2$.
    % or with $p=1-2d \in (0,1)$
    % \[
    % \sum_{k=1}^\infty \sin(k \om) k^{-p} = \om^{p-1} \Gamma(1-p) \cos\left( p \frac{\pi}{2}\right) + R(\om),
    % \]
    % where the remainder term $R(\om) \to C \in \RR$ as $\om \to 0^+$. 
\end{lemma}

\begin{proof}
    Write
    \begin{equation} \label{eq:lemma-aux-1}
    \begin{split}
        \int_0^\infty e^{iu \om} u^{2d-1} du - \sum_{k=1}^\infty e^{ik\om} k^{2d-1} &= \sum_{k=1}^\infty \left( \int_{k-1}^{k} e^{iu \om} u^{2d-1} du -  e^{ik\om} k^{2d-1}  \right) \\
        &=\sum_{k=1}^\infty \left( \int_{k-1}^{k} e^{iu\om} (u^{2d-1} - k^{2d-1})du  + k^{2d-1}  \left( \int_{k-1}^{k} e^{iu\om} du - e^{ik\om}  \right)   \right) .
    \end{split}
    \end{equation}
    Next, note that, by Taylor's expansion,
    \begin{equation}
        \int_{k-1}^{k} (u^{2d-1} - k^{2d-1}) du = k^{2d} \int_{1-1/k}^{1} (z^{2d-1} -1) dz \sim  -k^{2d-2} \frac{2d-1}{2},
    \end{equation}
    which implies,
    % \begin{equation} 
    %     \left| \sum_{k=1}^\infty \int_k^{k+1} e^{iu \om} (u^{2d-1} - k^{2d-1}) du  \right| \le \sum_{k=1}^\infty \int_k^{k+1}  (k^{2d-1} - u^{2d-1}) du = C \in \RR_+,
    % \end{equation}
    % and so, 
    from the bounded convergence theorem, as $\om \to 0^+$,
    \begin{equation} \label{eq:lemma-aux-2}
        \sum_{k=1}^\infty \int_{k-1}^{k} e^{iu \om} (u^{2d-1} - k^{2d-1}) du \to - C.
    \end{equation}
    Moreover, 
    \begin{equation}
        \int_{k-1}^{k} e^{iu\om} du - e^{ik\om} = \frac{e^{i\om k } - e^{i\om (k-1)}}{i\om} - e^{i\om k} = e^{i k \om} \frac{1 - e^{- i \om}   -i \om}{i \om}.
    \end{equation}
    Thus,
    \begin{equation} \label{eq:lemma-aux-3}
        \sum_{k=1}^\infty k^{2d-1}  \left( \int_k^{k+1} e^{iu\om} du - e^{ik\om}  \right) = \frac{1 - e^{- i \om}   -i \om}{i \om} \sum_{k=1}^\infty (k^{2d-1} e^{ik \om}) \sim  \om^{-2d+1} \Gamma(2d) e^{i \pi (\frac{1}{2} - d) } = o(1),
    \end{equation}
    where the last asymptotic relation holds from Proposition A.2.1 of \cite{pipiras_taqqu_2017}. 
    By combining \eqref{eq:lemma-aux-1}--\eqref{eq:lemma-aux-3},
    \begin{equation}
    \begin{split}
        \sum_{k=1}^\infty e^{ik\om} k^{2d-1} &=  \int_0^\infty e^{iu \om} u^{2d-1} du  \\
        &\quad-\sum_{k=1}^\infty  \int_{k-1}^{k} e^{iu\om} (u^{2d-1} - k^{2d-1})du  - \sum_{k=1}^\infty k^{2d-1}  \left( \int_{k-1}^{k} e^{iu\om} du - e^{ik\om}  \right)   \\
        &= \om^{-2d} \Gamma(2d) e^{i d \pi}  + R(\om),
    \end{split}
    \end{equation}
    where, as $\om \to 0^+$, $R(\om) \to C - \frac{1}{2d}$ and $C$ is given in \eqref{eq:lemma-aux-2}.
\end{proof}




